MTG: A Benchmark Suite for Multilingual Text Generation

We introduce MTG, a new benchmark suite for training and evaluating multilingual text generation. It is the first-proposed multilingual multiway text generation dataset with the largest human-annotated data (400k). It includes four generation tasks (story generation, question generation, title generation and text summarization) across five languages (English, German, French, Spanish and Chinese). The multiway setup enables testing knowledge transfer capabilities for a model across languages and tasks. Using MTG, we train and analyze several popular multilingual generation models from different aspects. Our benchmark suite fosters model performance enhancement with more human-annotated parallel data. It provides comprehensive evaluations with diverse generation scenarios. Code and data are available at \url{https://github.com/zide05/MTG}.

==> tabs/correlation.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \footnotesize
%   \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{lcccccccc}
    \toprule
    Correlation & Bleu  & R-1 & R-2 & R-L & BERTScore-P & BERTScore-R & BERTScore-F1 & Ensemble \\
    \midrule
    Pearson & 0.127  & 0.106  & 0.101  & 0.106  & 0.202  & 0.207  & 0.209  & \textbf{0.240 } \\
    Spearman & 0.139  & 0.057  & 0.037  & 0.058  & 0.135  & 0.155  & 0.148  & \textbf{0.211 } \\
    Kendall & 0.099  & 0.042  & 0.029  & 0.043  & 0.096  & 0.109  & 0.105  & \textbf{0.182 } \\
    \bottomrule
    \end{tabular}%
    % }
  \caption{The pearson correlation scores between automatic metric scores and human annotated scores (the average scores of grammar, fluency and relevance). R-* denote ROUGE-*.}
  \label{tab:correlation compare}%
\end{table*}%


==> tabs/cross.tex <==
% % Table generated by Excel2LaTeX from sheet 'Cross-lingual'
% \begin{table*}\footnotesize
% \renewcommand\arraystretch{1}
%   \centering
%     \begin{tabular}{clrrrrr}
%     \toprule
%     \textbf{Task} & \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{R-L}} & \multicolumn{1}{c}{\textbf{METEOR}} & \multicolumn{1}{c}{\textbf{BERTS}} & \multicolumn{1}{c}{\textbf{D-1}} \\
%     \midrule
%     \multirow{4}[2]{*}{SG} & M-BERT & 0 & 0 & 0 & 0 & 0 \\
%       & XLM & 2.26 & 15.32 & 0.124 & 0.713 & 0.954 \\
%       & mBART & 1.4 & 11.6 & 0.12 & 0.717 & 0.969 \\
%       & mT5 & 0 & 0 & 0 & 0 & 0 \\
%     \midrule
%     \multirow{4}[2]{*}{QG} & M-BERT & 0 & 0 & 0 & 0 & 0 \\
%       & XLM & 13.6 & 40.3 & 0.316 & 0.797 & 0.949 \\
%       & mBART & 7.4 & 25.3 & 0.254 & 0.782 & 0.975 \\
%       & mT5 & 0 & 0 & 0 & 0 & 0 \\
%     \midrule
%     \multirow{4}[2]{*}{TG} & M-BERT & 0 & 0 & 0 & 0 & 0 \\
%       & XLM & 0 & 0 & 0 & 0 & 0 \\
%       & mBART & 0 & 0 & 0 & 0 & 0 \\
%       & mT5 & 0 & 0 & 0 & 0 & 0 \\
%     \bottomrule
%     \end{tabular}%
%     \caption{Add caption}
%   \label{tab:addlabel}%
% \end{table*}%


% Table generated by Excel2LaTeX from sheet 'Cross-lingual'
\begin{table}\footnotesize
\renewcommand\arraystretch{0.8}
  \centering
    \begin{tabular}{clccc}
    \toprule
    \textbf{Task} & \multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{R-L}} & \multicolumn{1}{c}{\textbf{BERTScore}} & \multicolumn{1}{c}{\textbf{D-1}} \\
    \midrule
    \multirow{4}[2]{*}{SG} & M-BERT & 13.1 & 0.716 & 0.941 \\
      & XLM & 15.3 & 0.713 & 0.954 \\
      & mBART & 11.6 & 0.717 & 0.969 \\
      & mT5 & 15.6 & 0.741 & 0.973 \\
    \midrule
    \multirow{4}[2]{*}{QG} & M-BERT & 19.4 & 0.733 & 0.918 \\
      & XLM & 40.3 & 0.797 & 0.949 \\
      & mBART & 25.3 & 0.782 & 0.975 \\
      & mT5 & 31.3 & 0.804 & 0.972 \\
    \midrule
    \multirow{4}[2]{*}{TG} & M-BERT & 16.3 & 0.705 & 0.924 \\
      & XLM & 26.2 & 0.739 & 0.910 \\
      & mBART & 19.9 & 0.730 & 0.953 \\
      & mT5 & 25.3 & 0.748 & 0.935 \\
    \bottomrule
    \end{tabular}%
    \caption{Cross-lingual evaluation scenarios. We choose one metric for each type. The results are the average scores on the en->de, en->fr, en->es test set.}
  \label{tab:cross}%
\end{table}%



==> tabs/ensemble_choose.tex <==
% Table generated by Excel2LaTeX from sheet 'table for paper'
\begin{table*}[htbp]
  \centering
%   \footnotesize
\resizebox{0.97\textwidth}{!}{%
    \begin{tabular}{lccccccccc}
    \toprule
    \textbf{Human score} & \textbf{AdaBoost} & \textbf{Bagging} & \textbf{DecisionTree} & \textbf{ExtraTree} & \textbf{GradientBoosting} & \textbf{Kneighbors} & \textbf{Linear} & \textbf{RandomForest} & \textbf{SVR} \\
    \midrule
    Grammar & 0.425  & 0.401  & 0.317  & 0.204  & \textbf{0.434 } & 0.249  & 0.385  & 0.410  & 0.220  \\
    Fluency & 0.458  & 0.422  & 0.329  & 0.271  & \textbf{0.475 } & 0.261  & 0.421  & 0.420  & 0.204  \\
    Logical & 0.201  & 0.359  & 0.227  & 0.252  & 0.302  & 0.314  & 0.177  & \textbf{0.385 } & 0.311  \\
    Avg   & 0.386  & 0.493  & 0.353  & 0.297  & 0.456  & 0.362  & 0.359  & \textbf{0.510 } & 0.331  \\
    \bottomrule
    \end{tabular}%
    }
    \caption{The pearson correlation scores between different regressors and human-annotated scores. Avg means the adverage human-annotated score of Grammar, Fluency and Logical.}
  \label{tab:ensemble choose}%
\end{table*}%




==> tabs/extab/cross_old.tex <==
% Table generated by Excel2LaTeX from sheet 'Cross-lingual'
\begin{table*}\footnotesize
\renewcommand\arraystretch{0.6}
  \centering
    \begin{tabular}{cccrrrrr}
    \toprule
      &   &   & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{Distant-L} \\
      \midrule
    \multirow{12}[8]{*}{SG} & \multirow{3}[2]{*}{M-BERT} & en->de & 2.13 & 13.4 & 0.135 & 0.714 & 0.939 \\
      &   & en->fr & 1.21 & 12.7 & 0.201 & 0.719 & 0.949 \\
      &   & en->es & 1.69 & 13.1 & 0.115 & 0.714 & 0.934 \\
\cmidrule{2-8}      & \multirow{3}[2]{*}{XLM} & en->de & 2.14 & 14.7 & 0.090 & 0.705 & 0.977 \\
      &   & en->fr & 2.70 & 17.2 & 0.176 & 0.719 & 0.932 \\
      &   & en->es & 1.93 & 14.1 & 0.107 & 0.714 & 0.954 \\
\cmidrule{2-8}      & \multirow{3}[2]{*}{mBART} & en->de & 1.48 & 11.0 & 0.103 & 0.701 & 0.969 \\
      &   & en->fr & 1.43 & 12.7 & 0.164 & 0.727 & 0.977 \\
      &   & en->es & 1.25 & 11.2 & 0.094 & 0.723 & 0.961 \\
\cmidrule{2-8}      & \multirow{3}[2]{*}{mT5} & en->de & 3.33 & 15.2 & 0.138 & 0.733 & 0.978 \\
      &   & en->fr & 3.11 & 16.4 & 0.192 & 0.747 & 0.965 \\
      &   & en->es & 3.42 & 15.1 & 0.131 & 0.743 & 0.974 \\
    \midrule
    \multirow{12}[8]{*}{QG} & \multirow{3}[2]{*}{M-BERT} & en->de & 5.68 & 19.5 & 0.181 & 0.705 & 0.922 \\
      &   & en->fr & 4.96 & 19.1 & 0.239 & 0.730 & 0.914 \\
      &   & en->es & 5.43 & 19.6 & 0.278 & 0.764 & 0.917 \\
\cmidrule{2-8}      & \multirow{3}[2]{*}{XLM} & en->de & 9.18 & 35.3 & 0.239 & 0.770 & 0.967 \\
      &   & en->fr & 14.7 & 39.6 & 0.346 & 0.795 & 0.944 \\
      &   & en->es & 16.9 & 46.0 & 0.365 & 0.827 & 0.936 \\
\cmidrule{2-8}      & \multirow{3}[2]{*}{mBART} & en->de & 4.62 & 20.6 & 0.171 & 0.750 & 0.985 \\
      &   & en->fr & 8.10 & 25.6 & 0.277 & 0.772 & 0.967 \\
      &   & en->es & 9.55 & 29.7 & 0.313 & 0.823 & 0.973 \\
\cmidrule{2-8}      & \multirow{3}[2]{*}{mT5} & en->de & 8.81 & 27.2 & 0.231 & 0.776 & 0.983 \\
      &   & en->fr & 12.4 & 31.5 & 0.336 & 0.799 & 0.967 \\
      &   & en->es & 14.4 & 35.4 & 0.372 & 0.838 & 0.966 \\
    \midrule
    \multirow{12}[8]{*}{TG} & \multirow{3}[2]{*}{M-BERT} & en->de & 4.35 & 13.8 & 0.150 & 0.694 & 0.934 \\
      &   & en->fr & 3.35 & 13.2 & 0.145 & 0.696 & 0.926 \\
      &   & en->es & 6.60 & 22.00 & 0.231 & 0.726 & 0.912 \\
\cmidrule{2-8}      & \multirow{3}[2]{*}{XLM} & en->de & 6.96 & 21.5 & 0.194 & 0.716 & 0.938 \\
      &   & en->fr & 9.96 & 27.3 & 0.284 & 0.744 & 0.898 \\
      &   & en->es & 11.26 & 29.9 & 0.292 & 0.756 & 0.895 \\
\cmidrule{2-8}      & \multirow{3}[2]{*}{mBART} & en->de & 6.36 & 14.5 & 0.153 & 0.706 & 0.951 \\
      &   & en->fr & 8.39 & 21.6 & 0.213 & 0.738 & 0.958 \\
      &   & en->es & 9.85 & 23.6 & 0.250 & 0.748 & 0.949 \\
\cmidrule{2-8}      & \multirow{3}[2]{*}{mT5} & en->de & 8.38 & 20 & 0.201 & 0.728 & 0.964 \\
      &   & en->fr & 10.6 & 26.6 & 0.282 & 0.751 & 0.921 \\
      &   & en->es & 12.46 & 29.3 & 0.307 & 0.765 & 0.919 \\
    \bottomrule
    \end{tabular}%
    \caption{The whole results under the cross-lingual evaluation scenarios.}
  \label{tab:cross}%
\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Cross-lingual'
% \begin{tabular}{cc|c|ccc|cc}
% \toprule
%   &   &   & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{Distant-L} \\
% \bottomrule
% \end{tabular}%


==> tabs/extab/mono_m.tex <==
% % Table generated by Excel2LaTeX from sheet 'mono-m'
% \begin{table*}[htbp]
%   \renewcommand\arraystretch{0.6}
%   \centering
%   \footnotesize
%     \begin{tabular}{cclccccccc}
%     \toprule
%     \multirow{2}[2]{*}{\textbf{Task}} & \multirow{2}[2]{*}{\textbf{Model}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{Language}}} & \multicolumn{2}{c}{\textbf{N-gram-based}} & \multicolumn{3}{c}{\textbf{Embedding-based}} & \textbf{Others} & \textbf{Ours} \\
%           &       &       & \textbf{BLEU} & \textbf{ROUGE-L} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{BLEURT} & \textbf{Distant-1} & \textbf{Ensemble} \\
%     \midrule
%     \multirow{16}[8]{*}{SG} & \multirow{4}[2]{*}{M-BERT} & en->en & 2.73  & 19.4  & 0.102 & 0.886 & -0.812 & 0.92  & 3.69 \\
%           &       & de->de & 2.46  & 13.3  & 0.13  & 0.718 & -     & 0.946 & 3.226 \\
%           &       & fr->fr & 1.53  & 13.6  & 0.196 & 0.721 & -     & 0.935 & 3.28 \\
%           &       & es->es & 1.86  & 13.3  & 0.115 & 0.717 & -     & 0.955 & 3.178 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{XLM} & en->en & 3.06  & 19.9  & 0.091 & 0.877 & -0.756 & 0.962 & 3.753 \\
%           &       & de->de & 2.98  & 16.3  & 0.107 & 0.708 & -     & 0.973 & 3.336 \\
%           &       & fr->fr & 3.52  & 18.3  & 0.173 & 0.723 & -     & 0.959 & 3.398 \\
%           &       & es->es & 2.44  & 15    & 0.116 & 0.718 & -     & 0.962 & 3.32 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mBART} & en->en & 3.96  & 20.8  & 0.11  & 0.894 & -0.692 & 0.983 & 3.744 \\
%           &       & de->de & 3.23  & 14.7  & 0.131 & 0.731 & -     & 0.989 & 3.326 \\
%           &       & fr->fr & 3.89  & 16.3  & 0.197 & 0.749 & -     & 0.989 & 3.4 \\
%           &       & es->es & 3.64  & 14.8  & 0.131 & 0.741 & -     & 0.988 & 3.29 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mT5} & en->en & 2.51  & 17.7  & 0.099 & 0.889 & -0.755 & 0.981 & 3.687 \\
%           &       & de->de & 1.92  & 12.5  & 0.129 & 0.722 & -     & 0.971 & 3.271 \\
%           &       & fr->fr & 2.7   & 13.1  & 0.2   & 0.738 & -     & 0.962 & 3.331 \\
%           &       & es->es & 2.5   & 13    & 0.12  & 0.735 & -     & 0.974 & 3.212 \\
%     \midrule
%     \multirow{16}[8]{*}{QG} & \multirow{4}[2]{*}{M-BERT} & en->en & 13.03 & 38.4  & 0.192 & 0.89  & -0.431 & 0.895 & 3.924 \\
%           &       & de->de & 5.97  & 20.8  & 0.19  & 0.736 & -     & 0.915 & 3.305 \\
%           &       & fr->fr & 6.64  & 21.5  & 0.256 & 0.747 & -     & 0.909 & 3.427 \\
%           &       & es->es & 8.1   & 22.9  & 0.311 & 0.79  & -     & 0.928 & 3.613 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{XLM} & en->en & 20.18 & 45.3  & 0.231 & 0.912 & -0.259 & 0.961 & 4.043 \\
%           &       & de->de & 11.95 & 38.3  & 0.259 & 0.783 & -     & 0.974 & 3.682 \\
%           &       & fr->fr & 16.99 & 41.4  & 0.359 & 0.8   & -     & 0.951 & 3.753 \\
%           &       & es->es & 18.85 & 47    & 0.379 & 0.83  & -     & 0.95  & 3.872 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mBART} & en->en & 18.89 & 44.8  & 0.218 & 0.912 & -0.259 & 0.976 & 4.04 \\
%           &       & de->de & 11.29 & 28.3  & 0.234 & 0.781 & -     & 0.988 & 3.538 \\
%           &       & fr->fr & 13.99 & 31.8  & 0.324 & 0.789 & -     & 0.982 & 3.653 \\
%           &       & es->es & 15.82 & 34.5  & 0.365 & 0.831 & -     & 0.976 & 3.784 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mT5} & en->en & 19.45 & 44.8  & 0.223 & 0.912 & -0.273 & 0.973 & 4.039 \\
%           &       & de->de & 8.93  & 22.2  & 0.211 & 0.733 & -     & 0.956 & 3.399 \\
%           &       & fr->fr & 15.63 & 30.1  & 0.339 & 0.78  & -     & 0.955 & 3.624 \\
%           &       & es->es & 16.51 & 29.5  & 0.374 & 0.821 & -     & 0.957 & 3.737 \\
%     \midrule
%     \multirow{16}[8]{*}{TG} & \multirow{4}[2]{*}{M-BERT} & en->en & 14.84 & 36.3  & 0.204 & 0.882 & -0.527 & 0.915 & 3.896 \\
%           &       & de->de & 6.18  & 15.7  & 0.165 & 0.707 & -     & 0.892 & 3.122 \\
%           &       & fr->fr & 7.53  & 21.8  & 0.238 & 0.732 & -     & 0.898 & 3.404 \\
%           &       & es->es & 8.96  & 25.3  & 0.268 & 0.749 & -     & 0.898 & 3.507 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{XLM} & en->en & 15.86 & 35.4  & 0.209 & 0.887 & -0.523 & 0.963 & 3.923 \\
%           &       & de->de & 7.51  & 21.8  & 0.194 & 0.716 & -     & 0.932 & 3.367 \\
%           &       & fr->fr & 11.18 & 28.3  & 0.294 & 0.746 & -     & 0.901 & 3.554 \\
%           &       & es->es & 10.79 & 29    & 0.285 & 0.753 & -     & 0.9   & 3.595 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mBART} & en->en & 20.58 & 41.7  & 0.224 & 0.9   & -0.384 & 0.985 & 4.004 \\
%           &       & de->de & 8.62  & 21.7  & 0.19  & 0.73  & -     & 0.979 & 3.391 \\
%           &       & fr->fr & 10.95 & 28.4  & 0.261 & 0.755 & -     & 0.955 & 3.534 \\
%           &       & es->es & 12.18 & 30.8  & 0.296 & 0.766 & -     & 0.945 & 3.597 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mT5} & en->en & 14.31 & 33.1  & 0.187 & 0.883 & -0.533 & 0.974 & 3.879 \\
%           &       & de->de & 6.15  & 15.7  & 0.153 & 0.701 & -     & 0.95  & 3.256 \\
%           &       & fr->fr & 9.51  & 23.9  & 0.248 & 0.731 & -     & 0.934 & 3.458 \\
%           &       & es->es & 11.25 & 26.5  & 0.271 & 0.74  & -     & 0.922 & 3.503 \\
%     \bottomrule
%     \end{tabular}%
%     \caption{The whole results under the monolingual multitask evaluation scenarios.}
%   \label{tab:mono m all}%
% \end{table*}%

% Table generated by Excel2LaTeX from sheet 'mono-multitask'
\begin{table*}[htbp]
  \renewcommand\arraystretch{0.6}
  \centering
  \footnotesize
\resizebox{0.93\textwidth}{!}{
    \begin{tabular}{cclcccccc}
    \toprule
    \multirow{2}[1]{*}{\textbf{Task}} & \multirow{2}[1]{*}{\textbf{Model}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{\textbf{Language}}} & \multicolumn{3}{c}{\textbf{N-gram-based}} & \multicolumn{1}{l}{\textbf{Embedding-based}} & \textbf{Others} & \textbf{Ours} \\
          &       &       & \textbf{BLEU} & \textbf{ROUGE-L} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{Distant-1} & \textbf{Ensemble} \\
          \midrule
    \multirow{20}[6]{*}{SG} & \multirow{5}[1]{*}{mBERT} & en->en & 2.51  & 19.1  & 0.099 & 0.899 & 0.968 & 3.839 \\
          &       & de->de & 2.42  & 13.2  & 0.118 & 0.722 & 0.977 & 3.818 \\
          &       & fr->fr & 1.41  & 13.4  & 0.182 & 0.72  & 0.948 & 3.709 \\
          &       & es->es & 2.3   & 13.1  & 0.114 & 0.717 & 0.98  & 3.78 \\
          &       & zh->zh & 5.03  & 24.9  & -     & 0.66  & 1     & 2.176 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{XLM} & en->en & 3.25  & 19.8  & 0.105 & 0.894 & 0.967 & 3.836 \\
          &       & de->de & 3.05  & 25.2  & 0.14  & 0.728 & 0.972 & 3.783 \\
          &       & fr->fr & 4.08  & 25.5  & 0.191 & 0.741 & 0.946 & 3.702 \\
          &       & es->es & 3.42  & 24.9  & 0.13  & 0.736 & 0.968 & 3.781 \\
          &       & zh->zh & 5.52  & 25.5  & -     & 0.665 & 0.991 & 1.847 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{mBART} & en->en & 3.87  & 20.6  & 0.107 & 0.901 & 0.977 & 3.861 \\
          &       & de->de & 3.15  & 14.6  & 0.13  & 0.731 & 0.987 & 3.82 \\
          &       & fr->fr & 3.73  & 16.5  & 0.187 & 0.748 & 0.984 & 3.789 \\
          &       & es->es & 3.3   & 14.6  & 0.127 & 0.737 & 0.979 & 3.833 \\
          &       & zh->zh & 6.04  & 26.5  & -     & 0.672 & 0.999 & 2.129 \\
\cmidrule{2-9}          & \multirow{5}[1]{*}{mT5} & en->en & 2.33  & 17.7  & 0.097 & 0.896 & 0.979 & 3.823 \\
          &       & de->de & 2.26  & 13.2  & 0.134 & 0.725 & 0.97  & 3.772 \\
          &       & fr->fr & 2.51  & 12.7  & 0.194 & 0.739 & 0.972 & 3.705 \\
          &       & es->es & 2.41  & 13.1  & 0.119 & 0.736 & 0.979 & 3.783 \\
          &       & zh->zh & 4.04  & 24.3  & -     & 0.663 & 1     & 1.89 \\
          \midrule
    \multirow{20}[6]{*}{QG} & \multirow{5}[1]{*}{mBERT} & en->en & 18.5  & 44.8  & 0.223 & 0.906 & 0.959 & 4.071 \\
          &       & de->de & 8.41  & 25.3  & 0.226 & 0.765 & 0.947 & 3.798 \\
          &       & fr->fr & 7.63  & 23.3  & 0.271 & 0.757 & 0.943 & 3.728 \\
          &       & es->es & 11.5  & 26.4  & 0.36  & 0.81  & 0.957 & 3.821 \\
          &       & zh->zh & 14.86 & 36.3  & -     & 0.719 & 0.999 & 3.44 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{XLM} & en->en & 20.2  & 45.2  & 0.233 & 0.915 & 0.965 & 4.112 \\
          &       & de->de & 12.24 & 38.2  & 0.265 & 0.784 & 0.978 & 3.906 \\
          &       & fr->fr & 17.75 & 41.5  & 0.365 & 0.802 & 0.951 & 3.9 \\
          &       & es->es & 20.78 & 48.5  & 0.394 & 0.835 & 0.953 & 4.022 \\
          &       & zh->zh & 15.36 & 35.4  & -     & 0.722 & 0.996 & 2.592 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{mBART} & en->en & 19.63 & 44.8  & 0.223 & 0.915 & 0.971 & 4.114 \\
          &       & de->de & 12.36 & 30.2  & 0.252 & 0.786 & 0.987 & 3.92 \\
          &       & fr->fr & 14.56 & 32.5  & 0.332 & 0.792 & 0.982 & 3.904 \\
          &       & es->es & 18.05 & 37.3  & 0.392 & 0.838 & 0.976 & 3.966 \\
          &       & zh->zh & 18.07 & 39.7  & -     & 0.737 & 0.998 & 3.667 \\
\cmidrule{2-9}          & \multirow{5}[1]{*}{mT5} & en->en & 17.94 & 42.2  & 0.211 & 0.912 & 0.966 & 4.082 \\
          &       & de->de & 11.71 & 27    & 0.261 & 0.774 & 0.968 & 3.829 \\
          &       & fr->fr & 15.87 & 30.6  & 0.341 & 0.788 & 0.961 & 3.847 \\
          &       & es->es & 15.99 & 29.5  & 0.372 & 0.827 & 0.956 & 3.863 \\
          &       & zh->zh & 13.88 & 34.4  & -     & 0.707 & 0.998 & 3.601 \\
          \midrule
    \multirow{20}[6]{*}{TG} & \multirow{5}[1]{*}{mBERT} & en->en & 15.51 & 36.9  & 0.206 & 0.888 & 0.967 & 3.952 \\
          &       & de->de & 6.81  & 17    & 0.169 & 0.713 & 0.941 & 3.615 \\
          &       & fr->fr & 7.51  & 21.8  & 0.228 & 0.73  & 0.924 & 3.662 \\
          &       & es->es & 9.95  & 26.3  & 0.277 & 0.752 & 0.922 & 3.728 \\
          &       & zh->zh & 11.35 & 28.2  & -     & 0.671 & 0.993 & 2.466 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{XLM} & en->en & 15.74 & 35.4  & 0.212 & 0.891 & 0.967 & 3.953 \\
          &       & de->de & 8.07  & 22.4  & 0.202 & 0.72  & 0.95  & 3.649 \\
          &       & fr->fr & 11.87 & 29    & 0.302 & 0.75  & 0.91  & 3.682 \\
          &       & es->es & 12.71 & 30.8  & 0.302 & 0.761 & 0.904 & 3.717 \\
          &       & zh->zh & 13.82 & 27.3  & -     & 0.675 & 0.97  & 2.088 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{mBART} & en->en & 20.33 & 41.3  & 0.221 & 0.903 & 0.986 & 4.049 \\
          &       & de->de & 8.5   & 21.8  & 0.192 & 0.73  & 0.976 & 3.755 \\
          &       & fr->fr & 10.61 & 28    & 0.257 & 0.753 & 0.958 & 3.765 \\
          &       & es->es & 13.16 & 31.6  & 0.308 & 0.768 & 0.939 & 3.802 \\
          &       & zh->zh & 17.14 & 33.6  & -     & 0.7   & 0.988 & 2.811 \\
\cmidrule{2-9}          & \multirow{5}[1]{*}{mT5} & en->en & 14.56 & 34.9  & 0.187 & 0.891 & 0.979 & 3.953 \\
          &       & de->de & 7.74  & 18.1  & 0.177 & 0.712 & 0.96  & 3.635 \\
          &       & fr->fr & 9.85  & 24.5  & 0.243 & 0.738 & 0.942 & 3.675 \\
          &       & es->es & 11.52 & 27.2  & 0.272 & 0.751 & 0.928 & 3.712 \\
          &       & zh->zh & 10.78 & 24.5  & -     & 0.654 & 0.986 & 2.663 \\
          \midrule
    \multirow{20}[6]{*}{Summ} & \multirow{5}[1]{*}{mBERT} & en->en & 14.4  & 38.1  & 0.173 & 0.871 & 0.821 & 3.937 \\
          &       & de->de & 7.61  & 24.2  & 0.195 & 0.711 & 0.79  & 3.727 \\
          &       & fr->fr & 8.82  & 28.2  & 0.286 & 0.725 & 0.736 & 3.623 \\
          &       & es->es & 9.41  & 31.7  & 0.265 & 0.741 & 0.768 & 3.682 \\
          &       & zh->zh & 10.4  & 35.5  & -     & 0.694 & 0.906 & 3.214 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{XLM} & en->en & 15.7  & 37.7  & 0.191 & 0.878 & 0.779 & 3.948 \\
          &       & de->de & 7.93  & 28.5  & 0.187 & 0.712 & 0.801 & 3.665 \\
          &       & fr->fr & 11.31 & 34.4  & 0.282 & 0.743 & 0.742 & 3.58 \\
          &       & es->es & 11.45 & 35.4  & 0.278 & 0.743 & 0.731 & 3.552 \\
          &       & zh->zh & 13.11 & 36.2  & -     & 0.694 & 0.83  & 1.975 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{mBART} & en->en & 0.35  & 20.1  & 0.066 & 0.855 & 0.964 & 3.578 \\
          &       & de->de & 0.11  & 12.8  & 0.066 & 0.668 & 0.962 & 3.132 \\
          &       & fr->fr & 0.12  & 14.7  & 0.085 & 0.692 & 0.954 & 3.153 \\
          &       & es->es & 0.2   & 16.6  & 0.12  & 0.699 & 0.934 & 3.187 \\
          &       & zh->zh & 0.48  & 19.7  & -     & 0.64  & 0.979 & 2.751 \\
\cmidrule{2-9}          & \multirow{5}[1]{*}{mT5} & en->en & 8.06  & 32    & 0.124 & 0.871 & 0.85  & 3.85 \\
          &       & de->de & 8.43  & 30.1  & 0.181 & 0.725 & 0.855 & 3.691 \\
          &       & fr->fr & 8.33  & 29.9  & 0.188 & 0.724 & 0.859 & 3.695 \\
          &       & es->es & 8.42  & 30.2  & 0.218 & 0.725 & 0.856 & 3.697 \\
          &       & zh->zh & 6.41  & 27.7  & -     & 0.657 & 0.873 & 3.324 \\
          \bottomrule
    \end{tabular}%
    }
  \caption{The whole results under the monolingual multitask evaluation scenarios.}
  \label{tab:mono m all}%
\end{table*}%


==> tabs/extab/mono_old.tex <==
% Table generated by Excel2LaTeX from sheet 'in-language'
\begin{table*}\footnotesize
\renewcommand\arraystretch{0.6}
  \centering
    \begin{tabular}{cccrrrrrr}
    \toprule
    \multirow{2}[1]{*}{\textbf{Task}} & \multirow{2}[1]{*}{\textbf{Model}} & \multirow{2}[1]{*}{\textbf{Language}} & \multicolumn{3}{c}{\textbf{N-gram-based}} & \multicolumn{2}{c}{\textbf{Embedding-based}} & \multicolumn{1}{c}{\textbf{Others}} \\
      &   &   & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{ROUGE-L}} & \multicolumn{1}{c}{\textbf{METEOR}} & \multicolumn{1}{c}{\textbf{BERTScore}} & \multicolumn{1}{c}{\textbf{BLEURT}} & \multicolumn{1}{c}{\textbf{Distant-1}} \\
      \midrule
    \multirow{16}[6]{*}{SG} & \multirow{4}[1]{*}{M-BERT} & en & 2.44 & 18.1 & 0.105 & 0.885 & -0.771 & 0.930 \\
      &   & de & 1.39 & 11.8 & 0.125 & 0.704 & - & 0.918 \\
      &   & fr & 1.13 & 12.0 & 0.205 & 0.711 & - & 0.935 \\
      &   & es & 1.26 & 12.4 & 0.106 & 0.701 & - & 0.949 \\
    \cmidrule{2-9}  & \multirow{4}[2]{*}{XLM} & en & 3.17 & 20.4 & 0.092 & 0.878 & -0.747 & 0.960 \\
      &   & de & 2.50 & 15.8 & 0.101 & 0.705 & - & 0.962 \\
      &   & fr & 3.40 & 18.3 & 0.167 & 0.722 & - & 0.952 \\
      &   & es & 3.13 & 16.3 & 0.123 & 0.723 & - & 0.960 \\
    \cmidrule{2-9}  & \multirow{4}[2]{*}{mBART} & en & 4.09 & 21.4 & 0.112 & 0.894 & -0.683 & 0.980 \\
      &   & de & 3.63 & 15.3 & 0.135 & 0.733 & - & 0.989 \\
      &   & fr & 4.07 & 17.0 & 0.194 & 0.750 & - & 0.985 \\
      &   & es & 4.03 & 15.4 & 0.136 & 0.743 & - & 0.987 \\
    \cmidrule{2-9}  & \multirow{4}[1]{*}{mT5} & en & 1.75 & 16.6 & 0.090 & 0.886 & -0.807 & 0.980 \\
      &   & de & 1.39 & 11.4 & 0.116 & 0.719 & - & 0.955 \\
      &   & fr & 2.34 & 12.6 & 0.189 & 0.737 & - & 0.963 \\
      &   & es & 2.25 & 12.5 & 0.117 & 0.729 & - & 0.950 \\
    \midrule
    \multirow{16}[7]{*}{QG} & \multirow{4}[1]{*}{M-BERT} & en & 12.9 & 38.6 & 0.189 & 0.891 & -0.45 & 0.918 \\
      &   & de & 4.80 & 19.6 & 0.18 & 0.727 & - & 0.921 \\
      &   & fr & 5.00 & 18.5 & 0.252 & 0.737 & - & 0.934 \\
      &   & es & 6.28 & 21.2 & 0.286 & 0.791 & - & 0.939 \\
    \cmidrule{2-9}  & \multirow{4}[2]{*}{XLM} & en & 19.2 & 44.0 & 0.226 & 0.911 & -0.256 & 0.959 \\
      &   & de & 10.2 & 35.5 & 0.237 & 0.772 & - & 0.970 \\
      &   & fr & 16.5 & 39.9 & 0.351 & 0.794 & - & 0.944 \\
      &   & es & 19.2 & 47.0 & 0.376 & 0.829 & - & 0.948 \\
    \cmidrule{2-9}  & \multirow{4}[2]{*}{mBART} & en & 19.1 & 44.7 & 0.216 & 0.912 & -0.27 & 0.971 \\
      &   & de & 11.1 & 27.7 & 0.233 & 0.778 & - & 0.986 \\
      &   & fr & 14.8 & 32.5 & 0.327 & 0.797 & - & 0.982 \\
      &   & es & 16.6 & 34.6 & 0.368 & 0.831 & - & 0.972 \\
    \cmidrule{2-9}  & \multirow{4}[2]{*}{mT5} & en & 17.5 & 41.6 & 0.207 & 0.908 & -0.382 & 0.967 \\
      &   & de & 9.93 & 23.3 & 0.216 & 0.768 & - & 0.979 \\
      &   & fr & 13.0 & 25.3 & 0.312 & 0.772 & - & 0.964 \\
      &   & es & 15.9 & 28.5 & 0.354 & 0.825 & - & 0.956 \\
    \midrule
    \multirow{16}[8]{*}{TG} & \multirow{4}[2]{*}{M-BERT} & en & 9.64 & 27.5 & 0.167 & 0.838 & -0.742 & 0.914 \\
      &   & de & 3.34 & 11.6 & 0.132 & 0.678 & \multicolumn{1}{l}{-} & 0.887 \\
      &   & fr & 5.27 & 18.2 & 0.217 & 0.709 & \multicolumn{1}{l}{-} & 0.900 \\
      &   & es & 6.75 & 21.8 & 0.227 & 0.718 & \multicolumn{1}{l}{-} & 0.871 \\
    \cmidrule{2-9}  & \multirow{4}[2]{*}{XLM} & en & 12.6 & 31.7 & 0.186 & 0.879 & \multicolumn{1}{l}{-0.582} & 0.960 \\
      &   & de & 6.3 & 19.9 & 0.178 & 0.710 & \multicolumn{1}{l}{-} & 0.942 \\
      &   & fr & 9.3 & 25.8 & 0.271 & 0.739 & \multicolumn{1}{l}{-} & 0.907 \\
      &   & es & 9.6 & 27.2 & 0.263 & 0.747 & \multicolumn{1}{l}{-} & 0.897 \\
    \cmidrule{2-9}  & \multirow{4}[2]{*}{mBART} & en & 22.1 & 42.4 & 0.233 & 0.901 & -0.362 & 0.984 \\
      &   & de & 9.48 & 22.9 & 0.203 & 0.734 & - & 0.977 \\
      &   & fr & 12.3 & 29.4 & 0.282 & 0.759 & - & 0.949 \\
      &   & es & 13.8 & 32.1 & 0.315 & 0.770 & - & 0.939 \\
    \cmidrule{2-9}  & \multirow{4}[2]{*}{mT5} & en & 15.0 & 34.7 & 0.19331 & 0.888 & -0.505 & 0.975 \\
      &   & de & 7.35 & 17.4 & 0.17407 & 0.713 & - & 0.958 \\
      &   & fr & 10.3 & 24.8 & 0.25612 & 0.741 & - & 0.933 \\
      &   & es & 12.8 &  28.7 & 0.300  & 0.761  & - & 0.920 \\
    \bottomrule
    \end{tabular}%
  \caption{The whole results under the monolingual evaluation scenarios.}
  \label{tab:mono}%
\end{table*}%



==> tabs/extab/multi_m.tex <==
% % Table generated by Excel2LaTeX from sheet 'multi-m'
% \begin{table*}[htbp]
%   \renewcommand\arraystretch{0.6}
%   \centering
%   \footnotesize
%     \begin{tabular}{cclccccccc}
%     \toprule
%     \multirow{2}[2]{*}{\textbf{Task}} & \multirow{2}[2]{*}{\textbf{Model}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{Language}}} & \multicolumn{2}{c}{\textbf{N-gram-based}} & \multicolumn{3}{c}{\textbf{Embedding-based}} & \textbf{Others} & \textbf{Ours} \\
%           &       &       & \textbf{BLEU} & \textbf{ROUGE-L} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{BLEURT} & \textbf{Distant-1} & \textbf{Ensemble} \\
%     \midrule
%     \multirow{16}[8]{*}{SG} & \multirow{4}[2]{*}{M-BERT} & en->en & 2.8   & 19.9  & 0.105 & 0.887 & -0.78 & 0.918 & 3.709 \\
%           &       & de->de & 2.71  & 14.1  & 0.135 & 0.72  & -     & 0.944 & 3.234 \\
%           &       & fr->fr & 1.54  & 13.7  & 0.205 & 0.719 & -     & 0.935 & 3.274 \\
%           &       & es->es & 2.04  & 13.7  & 0.121 & 0.718 & -     & 0.952 & 3.18 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{XLM} & en->en & 2.69  & 19.8  & 0.087 & 0.876 & -0.761 & 0.966 & 3.759 \\
%           &       & de->de & 2.94  & 16.9  & 0.109 & 0.711 & -     & 0.967 & 3.35 \\
%           &       & fr->fr & 3.34  & 18    & 0.173 & 0.723 & -     & 0.956 & 3.403 \\
%           &       & es->es & 2.74  & 15.8  & 0.12  & 0.721 & -     & 0.97  & 3.354 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mBART} & en->en & 3.95  & 21.4  & 0.111 & 0.894 & -0.69 & 0.98  & 3.758 \\
%           &       & de->de & 3.26  & 15.1  & 0.135 & 0.731 & -     & 0.987 & 3.333 \\
%           &       & fr->fr & 3.65  & 16.1  & 0.191 & 0.748 & -     & 0.986 & 3.387 \\
%           &       & es->es & 3.96  & 15.1  & 0.136 & 0.742 & -     & 0.986 & 3.286 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mT5} & en->en & 3.09  & 19.9  & 0.106 & 0.892 & -0.72 & 0.97  & 3.738 \\
%           &       & de->de & 2.96  & 14.3  & 0.139 & 0.729 & -     & 0.973 & 3.317 \\
%           &       & fr->fr & 3.25  & 15.5  & 0.2   & 0.744 & -     & 0.959 & 3.369 \\
%           &       & es->es & 3.05  & 14.4  & 0.129 & 0.741 & -     & 0.968 & 3.234 \\
%     \midrule
%     \multirow{16}[8]{*}{QG} & \multirow{4}[2]{*}{M-BERT} & en->en & 17.68 & 44    & 0.224 & 0.902 & -0.285 & 0.925 & 4.008 \\
%           &       & de->de & 9.22  & 25.7  & 0.241 & 0.76  & -     & 0.943 & 3.469 \\
%           &       & fr->fr & 8.04  & 23.9  & 0.286 & 0.758 & -     & 0.931 & 3.499 \\
%           &       & es->es & 10.57 & 25.4  & 0.353 & 0.804 & -     & 0.94  & 3.683 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{XLM} & en->en & 18.16 & 43.6  & 0.224 & 0.909 & -0.303 & 0.956 & 4.03 \\
%           &       & de->de & 11.25 & 37.2  & 0.256 & 0.778 & -     & 0.974 & 3.675 \\
%           &       & fr->fr & 15.97 & 40    & 0.357 & 0.796 & -     & 0.94  & 3.744 \\
%           &       & es->es & 18.05 & 46.4  & 0.374 & 0.827 & -     & 0.942 & 3.865 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mBART} & en->en & 20.24 & 47.2  & 0.229 & 0.916 & -0.199 & 0.978 & 4.069 \\
%           &       & de->de & 12.52 & 30.6  & 0.254 & 0.789 & -     & 0.988 & 3.591 \\
%           &       & fr->fr & 15.17 & 33.7  & 0.332 & 0.798 & -     & 0.98  & 3.679 \\
%           &       & es->es & 17.46 & 36.9  & 0.387 & 0.838 & -     & 0.974 & 3.822 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mT5} & en->en & 21.4  & 47.3  & 0.238 & 0.916 & -0.206 & 0.971 & 4.068 \\
%           &       & de->de & 12.33 & 28.2  & 0.262 & 0.774 & -     & 0.978 & 3.559 \\
%           &       & fr->fr & 17.03 & 33.2  & 0.356 & 0.794 & -     & 0.968 & 3.668 \\
%           &       & es->es & 18.25 & 31.7  & 0.399 & 0.831 & -     & 0.966 & 3.781 \\
%     \midrule
%     \multirow{16}[8]{*}{TG} & \multirow{4}[2]{*}{M-BERT} & en->en & 15.34 & 36.3  & 0.207 & 0.885 & -0.501 & 0.941 & 3.916 \\
%           &       & de->de & 6.94  & 16    & 0.177 & 0.71  & -     & 0.919 & 3.214 \\
%           &       & fr->fr & 7.6   & 22.1  & 0.238 & 0.731 & -     & 0.907 & 3.404 \\
%           &       & es->es & 9.09  & 25.5  & 0.271 & 0.749 & -     & 0.913 & 3.497 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{XLM} & en->en & 14.88 & 35.2  & 0.208 & 0.887 & -0.514 & 0.962 & 3.922 \\
%           &       & de->de & 8.17  & 23    & 0.209 & 0.721 & -     & 0.937 & 3.392 \\
%           &       & fr->fr & 11.16 & 28.4  & 0.294 & 0.748 & -     & 0.901 & 3.557 \\
%           &       & es->es & 12.13 & 30.5  & 0.303 & 0.76  & -     & 0.901 & 3.62 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mBART} & en->en & 20.61 & 42    & 0.221 & 0.9   & -0.372 & 0.987 & 4.003 \\
%           &       & de->de & 8.76  & 22.3  & 0.193 & 0.731 & -     & 0.977 & 3.393 \\
%           &       & fr->fr & 11.08 & 28.8  & 0.258 & 0.756 & -     & 0.954 & 3.531 \\
%           &       & es->es & 13.17 & 32.1  & 0.312 & 0.77  & -     & 0.94  & 3.615 \\
% \cmidrule{2-10}          & \multirow{4}[2]{*}{mT5} & en->en & 16.46 & 36.1  & 0.205 & 0.888 & -0.475 & 0.975 & 3.921 \\
%           &       & de->de & 8.07  & 18.6  & 0.186 & 0.712 & -     & 0.953 & 3.315 \\
%           &       & fr->fr & 11    & 25.8  & 0.269 & 0.737 & -     & 0.934 & 3.504 \\
%           &       & es->es & 12.53 & 28.4  & 0.297 & 0.749 & -     & 0.922 & 3.544 \\
%     \bottomrule
%     \end{tabular}%
%     \caption{The whole results under the multilingual multitask evaluation scenarios.}
%   \label{tab:multi m all}%
% \end{table*}%


% Table generated by Excel2LaTeX from sheet 'multi-multitask'
\begin{table*}[htbp]
  \renewcommand\arraystretch{0.6}
  \centering
  \footnotesize
\resizebox{0.93\textwidth}{!}{
    \begin{tabular}{cclcccccc}
    \toprule
    \multirow{2}[1]{*}{\textbf{Task}} & \multirow{2}[1]{*}{\textbf{Model}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{\textbf{Language}}} & \multicolumn{3}{c}{\textbf{N-gram-based}} & \multicolumn{1}{l}{\textbf{Embedding-based}} & \textbf{Others} & \textbf{Ours} \\
          &       &       & \textbf{BLEU} & \textbf{ROUGE-L} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{Distant-1} & \textbf{Ensemble} \\
          \midrule
    \multirow{20}[6]{*}{SG} & \multirow{5}[1]{*}{mBERT} & en->en & 2.87  & 19.4  & 0.099 & 0.9   & 0.977 & 3.843 \\
          &       & de->de & 2.66  & 14.2  & 0.127 & 0.724 & 0.981 & 3.806 \\
          &       & fr->fr & 1.71  & 14    & 0.178 & 0.728 & 0.972 & 3.742 \\
          &       & es->es & 2.13  & 12.9  & 0.114 & 0.724 & 0.987 & 3.824 \\
          &       & zh->zh & 5.32  & 25.8  & -     & 0.668 & 0.999 & 2.203 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{XLM} & en->en & 2.65  & 19.1  & 0.101 & 0.894 & 0.969 & 3.825 \\
          &       & de->de & 3.12  & 24.5  & 0.138 & 0.729 & 0.976 & 3.811 \\
          &       & fr->fr & 3.83  & 25.3  & 0.187 & 0.741 & 0.938 & 3.69 \\
          &       & es->es & 2.82  & 23.8  & 0.127 & 0.735 & 0.958 & 3.754 \\
          &       & zh->zh & 5.62  & 26.2  & -     & 0.666 & 0.992 & 1.804 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{mBART} & en->en & 3.89  & 21    & 0.111 & 0.901 & 0.973 & 3.873 \\
          &       & de->de & 3.46  & 15.3  & 0.135 & 0.73  & 0.983 & 3.811 \\
          &       & fr->fr & 3.68  & 16.5  & 0.204 & 0.746 & 0.982 & 3.774 \\
          &       & es->es & 3.89  & 15.3  & 0.138 & 0.741 & 0.98  & 3.832 \\
          &       & zh->zh & 6.25  & 27    & -     & 0.672 & 0.995 & 2.312 \\
\cmidrule{2-9}          & \multirow{5}[1]{*}{mT5} & en->en & 2.68  & 18.7  & 0.102 & 0.897 & 0.979 & 3.84 \\
          &       & de->de & 2.42  & 13.2  & 0.131 & 0.727 & 0.98  & 3.794 \\
          &       & fr->fr & 2.83  & 14    & 0.197 & 0.741 & 0.968 & 3.718 \\
          &       & es->es & 2.85  & 13.9  & 0.127 & 0.738 & 0.973 & 3.781 \\
          &       & zh->zh & 5.16  & 25.8  & -     & 0.669 & 1     & 2.037 \\
          \midrule
    \multirow{20}[6]{*}{QG} & \multirow{5}[1]{*}{mBERT} & en->en & 18.29 & 44.7  & 0.228 & 0.907 & 0.96  & 4.08 \\
          &       & de->de & 9.36  & 26.8  & 0.243 & 0.771 & 0.979 & 3.871 \\
          &       & fr->fr & 8.96  & 25.6  & 0.29  & 0.768 & 0.945 & 3.758 \\
          &       & es->es & 10.86 & 25.7  & 0.355 & 0.809 & 0.961 & 3.809 \\
          &       & zh->zh & 15.4  & 36.9  & -     & 0.722 & 0.999 & 3.42 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{XLM} & en->en & 19.42 & 44.8  & 0.229 & 0.914 & 0.962 & 4.101 \\
          &       & de->de & 11.04 & 36.2  & 0.253 & 0.775 & 0.969 & 3.866 \\
          &       & fr->fr & 15.84 & 39.5  & 0.348 & 0.794 & 0.942 & 3.857 \\
          &       & es->es & 18.11 & 46.4  & 0.365 & 0.827 & 0.948 & 3.983 \\
          &       & zh->zh & 13.74 & 34.1  & -     & 0.711 & 0.994 & 2.568 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{mBART} & en->en & 21.19 & 47.1  & 0.234 & 0.92  & 0.973 & 4.147 \\
          &       & de->de & 12.9  & 31    & 0.256 & 0.79  & 0.989 & 3.936 \\
          &       & fr->fr & 15.27 & 33.5  & 0.339 & 0.797 & 0.979 & 3.918 \\
          &       & es->es & 17.65 & 36.9  & 0.39  & 0.84  & 0.973 & 3.964 \\
          &       & zh->zh & 17.42 & 39.7  & -     & 0.734 & 0.998 & 3.667 \\
\cmidrule{2-9}          & \multirow{5}[1]{*}{mT5} & en->en & 19.91 & 45.8  & 0.227 & 0.917 & 0.973 & 4.131 \\
          &       & de->de & 12.53 & 29.1  & 0.257 & 0.785 & 0.985 & 3.907 \\
          &       & fr->fr & 16.58 & 33.2  & 0.351 & 0.8   & 0.971 & 3.896 \\
          &       & es->es & 18.51 & 36.3  & 0.386 & 0.839 & 0.972 & 3.954 \\
          &       & zh->zh & 17.38 & 39    & -     & 0.732 & 0.999 & 3.686 \\
          \midrule
    \multirow{20}[6]{*}{TG} & \multirow{5}[1]{*}{mBERT} & en->en & 16.42 & 38.4  & 0.209 & 0.893 & 0.976 & 4 \\
          &       & de->de & 7.58  & 18.1  & 0.186 & 0.72  & 0.958 & 3.68 \\
          &       & fr->fr & 8.22  & 23.6  & 0.238 & 0.739 & 0.946 & 3.703 \\
          &       & es->es & 9.88  & 26.6  & 0.279 & 0.756 & 0.935 & 3.758 \\
          &       & zh->zh & 11.6  & 29.1  & -     & 0.675 & 0.993 & 2.515 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{XLM} & en->en & 13.07 & 33.7  & 0.193 & 0.885 & 0.948 & 3.894 \\
          &       & de->de & 6.51  & 21.1  & 0.196 & 0.711 & 0.924 & 3.579 \\
          &       & fr->fr & 9.61  & 26.6  & 0.28  & 0.738 & 0.889 & 3.63 \\
          &       & es->es & 10.62 & 28.9  & 0.279 & 0.75  & 0.882 & 3.662 \\
          &       & zh->zh & 11.12 & 24.6  & -     & 0.659 & 0.966 & 2.065 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{mBART} & en->en & 20.96 & 41.6  & 0.226 & 0.904 & 0.986 & 4.059 \\
          &       & de->de & 9.29  & 22.6  & 0.2   & 0.732 & 0.976 & 3.735 \\
          &       & fr->fr & 11.38 & 28.7  & 0.263 & 0.756 & 0.956 & 3.786 \\
          &       & es->es & 13.29 & 32    & 0.313 & 0.77  & 0.941 & 3.798 \\
          &       & zh->zh & 16.42 & 33.4  & -     & 0.7   & 0.989 & 2.831 \\
\cmidrule{2-9}          & \multirow{5}[1]{*}{mT5} & en->en & 15.11 & 35.6  & 0.191 & 0.893 & 0.98  & 3.967 \\
          &       & de->de & 8.12  & 18.9  & 0.181 & 0.718 & 0.966 & 3.663 \\
          &       & fr->fr & 10.35 & 25.2  & 0.259 & 0.744 & 0.941 & 3.7 \\
          &       & es->es & 12.13 & 28.3  & 0.285 & 0.757 & 0.928 & 3.742 \\
          &       & zh->zh & 13.46 & 28.3  & -     & 0.676 & 0.987 & 2.718 \\
          \midrule
    \multirow{20}[6]{*}{Summ} & \multirow{5}[1]{*}{mBERT} & en->en & 15.02 & 38.9  & 0.176 & 0.873 & 0.839 & 3.944 \\
          &       & de->de & 7.89  & 25.1  & 0.196 & 0.718 & 0.836 & 3.812 \\
          &       & fr->fr & 8.7   & 29.2  & 0.262 & 0.733 & 0.794 & 3.75 \\
          &       & es->es & 10.22 & 32.4  & 0.276 & 0.744 & 0.772 & 3.699 \\
          &       & zh->zh & 12    & 36.7  & -     & 0.698 & 0.874 & 3.357 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{XLM} & en->en & 15.72 & 37.2  & 0.192 & 0.875 & 0.755 & 3.919 \\
          &       & de->de & 7.54  & 27.9  & 0.187 & 0.704 & 0.752 & 3.592 \\
          &       & fr->fr & 10.67 & 32.9  & 0.278 & 0.735 & 0.722 & 3.539 \\
          &       & es->es & 10.89 & 33.9  & 0.27  & 0.735 & 0.715 & 3.522 \\
          &       & zh->zh & 10.98 & 33.2  & -     & 0.679 & 0.813 & 1.965 \\
\cmidrule{2-9}          & \multirow{5}[2]{*}{mBART} & en->en & 0.36  & 20    & 0.066 & 0.855 & 0.966 & 3.573 \\
          &       & de->de & 0.11  & 12.8  & 0.066 & 0.668 & 0.962 & 3.131 \\
          &       & fr->fr & 0.13  & 14.9  & 0.084 & 0.692 & 0.954 & 3.171 \\
          &       & es->es & 0.21  & 16.5  & 0.118 & 0.698 & 0.936 & 3.196 \\
          &       & zh->zh & 0.48  & 19.4  & -     & 0.638 & 0.979 & 2.683 \\
\cmidrule{2-9}          & \multirow{5}[1]{*}{mT5} & en->en & 8.28  & 33.1  & 0.127 & 0.875 & 0.877 & 3.894 \\
          &       & de->de & 3.9   & 20.8  & 0.129 & 0.696 & 0.865 & 3.577 \\
          &       & fr->fr & 3.96  & 24.8  & 0.172 & 0.72  & 0.857 & 3.583 \\
          &       & es->es & 5.23  & 27.1  & 0.208 & 0.725 & 0.823 & 3.587 \\
          &       & zh->zh & 8.19  & 31.5  & -     & 0.679 & 0.888 & 3.522 \\
          \bottomrule
    \end{tabular}%
    }
  \caption{The whole results under the multilingual multitask evaluation scenarios.}
  \label{tab:multi m all}%
\end{table*}%


==> tabs/extab/multi_old.tex <==
% Table generated by Excel2LaTeX from sheet 'in-language'
\begin{table*}\footnotesize
\renewcommand\arraystretch{0.6}
  \centering
    \begin{tabular}{cccrrrrrr}
    \toprule
    \multirow{2}[1]{*}{\textbf{Task}} & \multirow{2}[1]{*}{\textbf{Model}} & \multirow{2}[1]{*}{\textbf{Language}} & \multicolumn{3}{c}{\textbf{N-gram-based}} & \multicolumn{2}{c}{\textbf{Embedding-based}} & \multicolumn{1}{c}{\textbf{Others}} \\
      &   &   & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{ROUGE-L}} & \multicolumn{1}{c}{\textbf{METEOR}} & \multicolumn{1}{c}{\textbf{BERTScore}} & \multicolumn{1}{c}{\textbf{BLEURT}} & \multicolumn{1}{c}{\textbf{Distant-1}} \\
      \midrule
    \cmidrule{1-7}\cmidrule{9-9}    \multirow{16}[8]{*}{SG} & \multirow{4}[2]{*}{M-BERT} & en & 2.60 & 18.1 & 0.098 & 0.888 & -0.772 & 0.971 \\
          &   & de & 1.58 & 12.0 & 0.111 & 0.721 & - & 0.978 \\
          &   & fr & 1.01 & 12.0 & 0.188 & 0.714 & - & 0.971 \\
          &   & es & 1.63 & 11.7 & 0.099 & 0.707 & - & 0.972 \\
    \cmidrule{2-9}      & \multirow{4}[2]{*}{XLM} & en & 2.14 & 18.3 & 0.08 & 0.874 & -0.808 & 0.964 \\
          &   & de & 2.19 & 15.3 & 0.101 & 0.702 & - & 0.966 \\
          &   & fr & 2.84 & 17.4 & 0.168 & 0.721 & - & 0.957 \\
          &   & es & 2.70 & 14.9 & 0.118 & 0.719 & - & 0.97 \\
    \cmidrule{2-9}      & \multirow{4}[2]{*}{mBART} & en & 4.45 & 21.9 & 0.116 & 0.895 & -0.668 & 0.981 \\
          &   & de & 3.62 & 15.4 & 0.138 & 0.734 & - & 0.988 \\
          &   & fr & 4.31 & 16.5 & 0.202 & 0.749 & - & 0.988 \\
          &   & es & 4.33 & 15.8 & 0.141 & 0.743 & - & 0.986 \\
    \cmidrule{2-9}      & \multirow{4}[2]{*}{mT5} & en & 3.77 & 20.5 & 0.108 & 0.894 & -7.000 & 0.972 \\
          &   & de & 3.12 & 14.6 & 0.134 & 0.732 & - & 0.983 \\
          &   & fr & 3.61 & 16.5 & 0.188 & 0.748 & - & 0.965 \\
          &   & es & 3.56 & 15.2 & 0.135 & 0.744 & - & 0.972 \\
        \midrule
        \multirow{16}[8]{*}{QG} & \multirow{4}[2]{*}{M-BERT} & en & 14.8 & 39.2 & 0.194 & 0.891 & -0.468 & 0.918 \\
          &   & de & 6.09 & 21.1 & 0.188 & 0.733 & - & 0.953 \\
          &   & fr & 6.34 & 21.6 & 0.262 & 0.741 & - & 0.926 \\
          &   & es & 7.36 & 21.9 & 0.298 & 0.789 & - & 0.931 \\
    \cmidrule{2-9}      & \multirow{4}[2]{*}{XLM} & en & 19.0 & 44.4 & 0.222 & 0.910 & -0.289 & 0.955 \\
          &   & de & 9.81 & 35.8 & 0.238 & 0.770 & - & 0.972 \\
          &   & fr & 16.2 & 40.3 & 0.351 & 0.797 & - & 0.946 \\
          &   & es & 19.0 & 47.3 & 0.375 & 0.830 & - & 0.942 \\
    \cmidrule{2-9}      & \multirow{4}[2]{*}{mBART} & en & 19.7 & 45.7 & 0.223 & 0.914 & -0.236 & 0.974 \\
          &   & de & 11.9 & 29.0 & 0.245 & 0.782 & - & 0.986 \\
          &   & fr & 14.8 & 32.6 & 0.327 & 0.793 & - & 0.978 \\
          &   & es & 16.4 & 34.5 & 0.366 & 0.832 & - & 0.972 \\
    \cmidrule{2-9}      & \multirow{4}[2]{*}{mT5} & en & 19.9 & 45.9 & 0.227 & 0.914 & -0.241 & 0.974 \\
          &   & de & 12.7 & 29.6 & 0.259 & 0.787 & - & 0.985 \\
          &   & fr & 16.2 & 32.7 & 0.343 & 0.799 & - & 0.970 \\
          &   & es & 18.8 & 36.8 & 0.390 & 0.839 & - & 0.970 \\
        \midrule
        \multirow{16}[8]{*}{TG} & \multirow{4}[2]{*}{M-BERT} & en & 9.88 & 28.1 & 0.164 & 0.848 & -0.736 & 0.931 \\
          &   & de & 3.83 & 12.1 & 0.137 & 0.681 & - & 0.909 \\
          &   & fr & 5.43 & 18.6 & 0.207 & 0.709 & - & 0.913 \\
          &   & es & 6.47 & 21.5 & 0.222 & 0.719 & - & 0.895 \\
    \cmidrule{2-9}      & \multirow{4}[2]{*}{XLM} & en & 12.08 & 32.2 & 0.191 & 0.88 & -0.579 & 0.956 \\
          &   & de & 6.03 & 20.3 & 0.184 & 0.69 & - & 0.935 \\
          &   & fr & 9.51 & 26.6 & 0.279 & 0.741 & - & 0.897 \\
          &   & es & 11 & 29.5 & 0.284 & 0.755 & - & 0.889 \\
    \cmidrule{2-9}      & \multirow{4}[2]{*}{mBART} & en & 21.2 & 42 & 0.231 & 0.901 & -0.345 & 0.984 \\
          &   & de & 9.42 & 22.7 & 0.202 & 0.734 & - & 0.973 \\
          &   & fr & 11.9 & 29.1 & 0.276 & 0.758 & - & 0.949 \\
          &   & es & 13.8 & 32.1 & 0.317 & 0.771 & - & 0.935 \\
    \cmidrule{2-9}      & \multirow{4}[2]{*}{mT5} & en & 17.0 & 37.1 & 0.214 & 0.893 & -0.448 & 0.976 \\
          &   & de & 8.21 & 18.8 & 0.193 & 0.72 & - & 0.954 \\
          &   & fr & 11.31 & 26.3 & 0.276 & 0.748 & - & 0.934 \\
          &   & es & 12.76 & 28.7 & 0.3 & 0.761 & - & 0.92 \\
    \bottomrule
    \end{tabular}%
  \caption{The whole results under the multilingual evaluation scenarios.}
  \label{tab:multi}%
\end{table*}%


==> tabs/extab/zero_old.tex <==
% Table generated by Excel2LaTeX from sheet 'Cross-lingual'
\begin{table*}\footnotesize
\renewcommand\arraystretch{0.6}
  \centering
    \begin{tabular}{cccrrrrr}
    \toprule
      &   &   & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{Distant-L} \\
      \midrule
        \multirow{12}[7]{*}{SG} & \multirow{3}[1]{*}{M-BERT} & de & 0.04 & 2.8 & 0.053 & 0.694 & 0.939 \\
      &   & fr & 0.04 & 3.7 & 0.05 & 0.706 & 0.942 \\
      &   & es & 0.04 & 3.1 & 0.04 & 0.708 & 0.941 \\
    \cmidrule{2-8}  & \multirow{3}[2]{*}{XLM} & de & 0.314 & 7.88 & 0.051 & 0.675 & 0.893 \\
      &   & fr & 0.712 & 10.5 & 0.094 & 0.695 & 0.899 \\
      &   & es & 0.347 & 8.84 & 0.058 & 0.692 & 0.884 \\
    \cmidrule{2-8}  & \multirow{3}[2]{*}{mBART} & de & 0.082 & 3.66 & 0.039 & 0.681 & 0.907 \\
      &   & fr & 0.066 & 4.30 & 0.037 & 0.689 & 0.908 \\
      &   & es & 0.060 & 3.92 & 0.038 & 0.691 & 0.897 \\
    \cmidrule{2-8}  & \multirow{3}[2]{*}{mT5} & de & 0.071 & 2.71 & 0.050 & 0.697 & 0.980 \\
      &   & fr & 0.040 & 3.79 & 0.044 & 0.708 & 0.979 \\
      &   & es & 0.041 & 3.30 & 0.038 & 0.711 & 0.980 \\
    \midrule
    \multirow{12}[8]{*}{QG} & \multirow{3}[2]{*}{M-BERT} & de & 0.63 & 4.1 & 0.067 & 0.770 & 0.925 \\
      &   & fr & 0.57 & 3.00 & 0.057 & 0.729 & 0.924 \\
      &   & es & 0.47 & 2.20 & 0.054 & 0.745 & 0.924 \\
    \cmidrule{2-8}  & \multirow{3}[2]{*}{XLM} & de & 2.14 & 19.89 & 0.119 & 0.724 & 0.927 \\
      &   & fr & 2.94 & 18.99 & 0.121 & 0.738 & 0.940 \\
      &   & es & 3.53 & 19.83 & 0.137 & 0.754 & 0.942 \\
    \cmidrule{2-8}  & \multirow{3}[2]{*}{mBART} & de & 1.21 & 6.04 & 0.079 & 0.735 & 0.977 \\
      &   & fr & 1.01 & 6.60 & 0.062 & 0.742 & 0.978 \\
      &   & es & 0.82 & 3.42 & 0.072 & 0.758 & 0.974 \\
    \cmidrule{2-8}  & \multirow{3}[2]{*}{mT5} & de & 1.51 & 5.58 & 0.084 & 0.739 & 0.971 \\
      &   & fr & 1.22 & 5.09 & 0.067 & 0.745 & 0.972 \\
      &   & es & 1.06 & 3.87 & 0.073 & 0.761 & 0.971 \\
    \midrule
    \multirow{12}[8]{*}{TG} & \multirow{3}[2]{*}{M-BERT} & de & 2.52 & 7.8 & \multicolumn{1}{r}{0.107} & 0.651 & 0.9 \\
      &   & fr & 1.81 & 6.9 & 0.104 & 0.658 & 0.916 \\
      &   & es & 1.74 & 6.8 & 0.106 & 0.666 & 0.906 \\
    \cmidrule{2-8}  & \multirow{3}[2]{*}{XLM} & de & 3.39 & 13.8 & 0.132 & 0.677 & 0.885 \\
      &   & fr & 3.27 & 13.2 & 0.131 & 0.690 & 0.885 \\
      &   & es & 3.51 & 14.2 & 0.135 & 0.697 & 0.878 \\
    \cmidrule{2-8}  & \multirow{3}[2]{*}{mBART} & de & 5.66 & 14.6 & 0.148 & 0.705 & 0.971 \\
      &   & fr & 3.91 & 12.9 & 0.131 & 0.710 & 0.978 \\
      &   & es & 4.07 & 12.4 & 0.155 & 0.718 & 0.969 \\
    \cmidrule{2-8}  & \multirow{3}[2]{*}{mT5} & de & 5.23 & 12.2 & 0.131 & 0.692 & 0.967 \\
      &   & fr & 3.92 & 10.8 & 0.118 & 0.702 & 0.975 \\
      &   & es & 4.00 & 10.65 & 0.135 & 0.710 & 0.967 \\
    \bottomrule
    \end{tabular}%
    \caption{The whole results under the zero-shot evaluation scenarios.}
  \label{tab:zero}%
\end{table*}%



==> tabs/human.tex <==
% Table generated by Excel2LaTeX from sheet 'Human evaluation'
\begin{table}\footnotesize
\renewcommand\arraystretch{0.7}
  \centering
    \begin{tabular}{clccc}
    \toprule
    \textbf{Setting} & \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Gram.}} & \multicolumn{1}{c}{\textbf{Flu.}} & \multicolumn{1}{c}{\textbf{Rel.}} \\
    \midrule
    \multirow{4}[2]{*}{Monolingual} & M-BERT & 4.30 & 4.43 & 3.91 \\
      & XLM & 4.44 & 4.65 & 4.18 \\
      & mBART & \textbf{4.59} & \textbf{4.70} & \textbf{4.34} \\
      & mT5 & 4.53 & 4.63 & 3.96 \\
    \midrule
    \multirow{4}[2]{*}{Multilingual} & M-BERT & 3.85 & 3.95 & 3.94 \\
      & XLM & 3.97 & 3.88 & 3.98 \\
      & mBART & 3.99 & 3.95 & \textbf{4.13} \\
      & mT5 & \textbf{4.00} & \textbf{4.03} & 4.10 \\
    \midrule
    \multirow{4}[2]{*}{Cross-lingual} & M-BERT & 3.80 & 3.78 & 3.47 \\
      & XLM & 3.99 & 3.86 & 3.63 \\
      & mBART & 3.51 & 3.41 & 3.20 \\
      & mT5 & \textbf{4.19} & \textbf{4.08} & \textbf{3.87} \\
    \midrule
    \multirow{4}[2]{*}{Zero-shot} & M-BERT & 1.00 & 1.00 & 1.00 \\
      & XLM & \textbf{2.32} & \textbf{2.19} & \textbf{1.91} \\
      & mBART & 1.00 & 1.00 & 1.00 \\
      & mT5 & 1.00 & 1.00 & 1.00 \\
    \bottomrule
    \end{tabular}%
  \caption{Human evaluation on SG task under four evaluation settings. The score is 1-5 with 5 is the best. It is the average score on four languages. `Gram.', `Flu.', `Rel.' indicates \textbf{Grammar}, \textbf{Fluency} and \textbf{Relevance} respectively. The bolded results are the best among four models. }
  \label{tab:human}%
\end{table}%


==> tabs/human2.tex <==
% % Table generated by Excel2LaTeX from sheet 'humaneval'
% \begin{table}\footnotesize
% \renewcommand\arraystretch{0.7}
%   \centering
%     \begin{tabular}{clccc}
%     \toprule
%     \textbf{Setting} & \multicolumn{1}{c}{\textbf{Model}} & \textbf{Gram.} & \textbf{Flu.} & \textbf{Rel.} \\
%     \midrule
%     \multirow{4}[2]{*}{Mono} & M-BERT & 3.89  & 3.93  & 3.55  \\
%           & XLM   & \textbf{4.37 } & \textbf{4.40 } & \textbf{4.13 } \\
%           & mBART & 4.02  & 4.03  & 3.83  \\
%           & mT5   & 4.18  & 4.17  & 4.05  \\
%     \midrule
%     \multirow{4}[2]{*}{Multi} & M-BERT & 3.89  & 3.78  & 3.70  \\
%           & XLM   & \textbf{4.03 } & \textbf{3.99 } & \textbf{3.84 } \\
%           & mBART & 3.96  & 3.72  & 3.58  \\
%           & mT5   & 3.84  & 3.74  & 3.72  \\
%     \midrule
%     \multirow{4}[2]{*}{Cross} & M-BERT & \textbf{3.82 } & \textbf{3.90 } & \textbf{3.94 } \\
%           & XLM   & 3.64  & 3.64  & 3.69  \\
%           & mBART & 3.68  & 3.64  & 3.70  \\
%           & mT5   & 3.72  & 3.58  & 3.81  \\
%     \midrule
%     \multirow{4}[2]{*}{Zero} & M-BERT & 2.47  & 1.76  & 1.67  \\
%           & XLM   & 3.16  & 2.69  & 2.72  \\
%           & mBART & 3.31  & 3.00  & 3.18  \\
%           & mT5   & \textbf{3.41 } & \textbf{3.22 } & \textbf{3.20 } \\
%     \bottomrule
%     \end{tabular}%
%     \caption{Human evaluation on TG task under four evaluation settings. The score is 1-5 with 5 is the best. It is the average score on four languages. `Gram.', `Flu.', `Rel.' indicates \textbf{Grammar}, \textbf{Fluency} and \textbf{Relevance} respectively. The bolded results are the best among four models. The full results are included in the appendix.}
%   \label{tab:human}%
% \end{table}%


% Table generated by Excel2LaTeX from sheet 'humaneval'
\begin{table}[htbp]
  \footnotesize
  \renewcommand\arraystretch{0.7}
  \centering
  \resizebox{0.38\textwidth}{!}{
    \begin{tabular}{rlccc}
    \toprule
    \multicolumn{1}{l}{\textbf{Setting}} & \textbf{Model} & \textbf{Gram.} & \textbf{Flu.} & \textbf{Rel.} \\
    \midrule
    \multicolumn{1}{l}{Mono} & M-BERT & 4.53  & 4.53  & 2.96  \\
          & XLM   & 4.47  & 4.49  & 3.05  \\
          & mBART & 4.66  & 4.69  & 3.03  \\
          & mT5   & \textbf{4.71 } & \textbf{4.78 } & \textbf{3.21 } \\
    \midrule
    \multicolumn{1}{l}{Multi} & M-BERT & 4.59  & 4.54  & 2.97  \\
          & XLM   & 4.53  & 4.53  & 3.07  \\
          & mBART & 4.69  & 4.67  & 3.06  \\
          & mT5   & \textbf{4.85 } & \textbf{4.87 } & \textbf{3.79 } \\
    \midrule
    \multicolumn{1}{l}{Cross} & M-BERT & 4.13  & 4.18  & 2.48  \\
          & XLM   & 4.15  & 4.13  & 2.52  \\
          & mBART & 4.30  & 4.30  & 2.70  \\
          & mT5   & \textbf{4.83 } & \textbf{4.93 } & \textbf{3.63 } \\
    \midrule
    \multicolumn{1}{l}{Zero} & M-BERT & 3.38  & 4.11  & 2.92  \\
          & XLM   & 3.27  & 4.06  & 3.15  \\
          & mBART & 3.35  & 4.26  & 3.18  \\
          & mT5   & \textbf{4.71 } & \textbf{4.85 } & \textbf{3.86 } \\
    \bottomrule
    \end{tabular}%
  }
  \caption{Human evaluation on QG task under four evaluation settings. The score is 1-5 with 5 is the best. It is the average score on four languages. `Gram.', `Flu.', `Rel.' indicates \textbf{Grammar}, \textbf{Fluency} and \textbf{Relevance} respectively. The bolded results are the best among four models. The full results are included in the appendix.}
  \label{tab:human}%
\end{table}%


==> tabs/human_qg.tex <==
% % Table generated by Excel2LaTeX from sheet 'humaneval'
% \begin{table}\footnotesize
% \renewcommand\arraystretch{0.7}
%   \centering
%     \begin{tabular}{clccc}
%     \toprule
%     \textbf{Setting} & \multicolumn{1}{c}{\textbf{Model}} & \textbf{Gram.} & \textbf{Flu.} & \textbf{Rel.} \\
%     \midrule
%     \multirow{4}[2]{*}{Mono} & M-BERT & 4.30  & 4.47  & 4.06  \\
%           & XLM   & 4.53  & 4.56  & 4.00  \\
%           & mBART & \textbf{4.65 } & \textbf{4.69 } & \textbf{4.14 } \\
%           & mT5   & 4.51  & 4.63  & 4.09  \\
%     \midrule
%     \multirow{4}[2]{*}{Multi} & M-BERT & \textbf{4.31 } & 4.38  & 4.22  \\
%           & XLM   & 4.20  & \textbf{4.39 } & \textbf{4.43 } \\
%           & mBART & 4.22  & 4.34  & 4.31  \\
%           & mT5   & 4.12  & 4.13  & 4.15  \\
%     \midrule
%     \multirow{4}[2]{*}{Mono-M} & M-BERT & \textbf{4.23 } & 4.37  & \textbf{3.76 } \\
%           & XLM   & 4.16  & 4.32  & 3.60  \\
%           & mBART & 4.13  & 4.38  & 3.51  \\
%           & mT5   & 4.18  & \textbf{4.44 } & 3.67  \\
%     \midrule
%     \multirow{4}[2]{*}{Multi-M} & M-BERT & \textbf{4.32 } & 4.42  & 3.78  \\
%           & XLM   & 4.31  & 4.41  & 3.78  \\
%           & mBART & 4.18  & 4.38  & 3.59  \\
%           & mT5   & 4.20  & \textbf{4.48 } & \textbf{3.79 } \\
%     \midrule
%     \multirow{4}[2]{*}{Cross} & M-BERT & \textbf{4.38 } & \textbf{4.56 } & \textbf{4.28 } \\
%           & XLM   & 4.09  & 4.19  & 4.19  \\
%           & mBART & 3.97  & 4.06  & 3.97  \\
%           & mT5   & 4.26  & 4.28  & 4.12  \\
%     \midrule
%     \multirow{4}[2]{*}{Zero} & M-BERT & 2.07  & 2.10  & 2.12  \\
%           & XLM   & 2.04  & 1.98  & 1.98  \\
%           & mBART & 2.07  & 2.04  & 2.04  \\
%           & mT5   & \textbf{2.19 } & \textbf{2.21 } & \textbf{2.22 } \\
%     \bottomrule
%     \end{tabular}%
%     \caption{Human evaluation on QG task under four evaluation settings. The score is 1-5 with 5 is the best. It is the average score on four languages. `Gram.', `Flu.', `Rel.' indicates \textbf{Grammar}, \textbf{Fluency} and \textbf{Relevance} respectively.}
%   \label{tab:human qg}%
% \end{table}%

% Table generated by Excel2LaTeX from sheet 'humaneval'
\begin{table}[htbp]
  \footnotesize
  \renewcommand\arraystretch{0.7}
  \centering
    \begin{tabular}{rlccc}
    \toprule
    \multicolumn{1}{l}{\textbf{Setting}} & \textbf{Model} & \textbf{Gram.} & \textbf{Flu.} & \textbf{Rel.} \\
    \midrule
    \multicolumn{1}{l}{Mono} & M-BERT & 4.53  & 4.53  & 2.96  \\
          & XLM   & 4.47  & 4.49  & 3.05  \\
          & mBART & 4.66  & 4.69  & 3.03  \\
          & mT5   & \textbf{4.71 } & \textbf{4.78 } & \textbf{3.21 } \\
    \midrule
    \multicolumn{1}{l}{Multi} & M-BERT & 4.59  & 4.54  & 2.97  \\
          & XLM   & 4.53  & 4.53  & 3.07  \\
          & mBART & 4.69  & 4.67  & 3.06  \\
          & mT5   & \textbf{4.85 } & \textbf{4.87 } & \textbf{3.79 } \\
    \midrule
    \multicolumn{1}{l}{Mono-M} & M-BERT & 4.52  & 4.51  & 2.15  \\
          & XLM   & 4.69  & 4.67  & 2.48  \\
          & mBART & 4.67  & 4.73  & 2.27  \\
          & mT5   & \textbf{4.74 } & \textbf{4.81 } & \textbf{3.58 } \\
    \midrule
    \multicolumn{1}{l}{Multi-M} & M-BERT & 4.61  & 4.55  & 2.25  \\
          & XLM   & 4.58  & 4.50  & 2.63  \\
          & mBART & 4.71  & 4.66  & 2.63  \\
          & mT5   & \textbf{4.75 } & \textbf{4.87 } & \textbf{4.35 } \\
    \midrule
    \multicolumn{1}{l}{Cross} & M-BERT & 4.13  & 4.18  & 2.48  \\
          & XLM   & 4.15  & 4.13  & 2.52  \\
          & mBART & 4.30  & 4.30  & 2.70  \\
          & mT5   & \textbf{4.83 } & \textbf{4.93 } & \textbf{3.63 } \\
    \midrule
    \multicolumn{1}{l}{Zero} & M-BERT & 3.38  & 4.11  & 2.92  \\
          & XLM   & 3.27  & 4.06  & 3.15  \\
          & mBART & 3.35  & 4.26  & 3.18  \\
          & mT5   & \textbf{4.71 } & \textbf{4.85 } & \textbf{3.86 } \\
    \bottomrule
    \end{tabular}%
  \caption{Human evaluation on QG task under four evaluation settings. The score is 1-5 with 5 is the best. It is the average score on four languages. `Gram.', `Flu.', `Rel.' indicates \textbf{Grammar}, \textbf{Fluency} and \textbf{Relevance} respectively.}
  \label{tab:human qg}%
\end{table}%



==> tabs/human_sg.tex <==
% Table generated by Excel2LaTeX from sheet 'humaneval'
\begin{table}\footnotesize
\renewcommand\arraystretch{0.7}
  \centering
    \begin{tabular}{clccc}
    \toprule
    \textbf{Setting} & \multicolumn{1}{c}{\textbf{Model}} & \textbf{Gram.} & \textbf{Flu.} & \textbf{Rel.} \\
    \midrule
    \multirow{4}[2]{*}{Mono} & M-BERT & 4.52  & 4.55  & 4.14  \\
          & XLM   & \textbf{4.56 } & 4.53  & 4.08  \\
          & mBART & 4.39  & 4.59  & 3.94  \\
          & mT5   & 4.40  & \textbf{4.73 } & \textbf{4.22 } \\
    \midrule
    \multirow{4}[2]{*}{Multi} & M-BERT & 3.70  & 3.62  & 3.91  \\
          & XLM   & 4.00  & \textbf{4.09 } & \textbf{4.16 } \\
          & mBART & 4.04  & 4.04  & 4.08  \\
          & mT5   & \textbf{4.07 } & 4.06  & 4.03  \\
    \midrule
    \multirow{4}[2]{*}{Mono-M} & M-BERT & 4.52  & 4.63  & \textbf{3.81 } \\
          & XLM   & 4.48  & 4.63  & 3.71  \\
          & mBART & \textbf{4.53 } & 4.63  & 3.62  \\
          & mT5   & 4.50  & 4.59  & 3.73  \\
    \midrule
    \multirow{4}[2]{*}{Multi-M} & M-BERT & 4.47  & 4.58  & \textbf{3.90 } \\
          & XLM   & 4.53  & 4.63  & 3.80  \\
          & mBART & 4.43  & \textbf{4.66 } & 3.61  \\
          & mT5   & 4.53  & 4.63  & 3.67  \\
    \midrule
    \multirow{4}[2]{*}{Cross} & M-BERT & 3.76  & 3.67  & 3.47  \\
          & XLM   & 3.91  & 3.79  & 3.59  \\
          & mBART & \textbf{3.94 } & \textbf{3.86 } & 3.50  \\
          & mT5   & 3.88  & 3.81  & \textbf{3.61 } \\
    \midrule
    \multirow{4}[2]{*}{Zero} & M-BERT & 1.36  & 1.28  & 1.23  \\
          & XLM   & \textbf{1.47 } & \textbf{1.47 } & \textbf{1.36 } \\
          & mBART & 1.16  & 1.12  & 1.07  \\
          & mT5   & 1.34  & 1.32  & 1.26  \\
    \bottomrule
    \end{tabular}%
    \caption{Human evaluation on SG task under four evaluation settings. The score is 1-5 with 5 is the best. It is the average score on four languages. `Gram.', `Flu.', `Rel.' indicates \textbf{Grammar}, \textbf{Fluency} and \textbf{Relevance} respectively.}
  \label{tab:human sg}%
\end{table}%



==> tabs/human_tg.tex <==
% Table generated by Excel2LaTeX from sheet 'humaneval'
\begin{table}\footnotesize
\renewcommand\arraystretch{0.7}
  \centering
    \begin{tabular}{clccc}
    \toprule
    \textbf{Setting} & \multicolumn{1}{c}{\textbf{Model}} & \textbf{Gram.} & \textbf{Flu.} & \textbf{Rel.} \\
    \midrule
    \multirow{4}[2]{*}{Mono} & M-BERT & 3.89  & 3.93  & 3.55  \\
          & XLM   & \textbf{4.37 } & \textbf{4.40 } & \textbf{4.13 } \\
          & mBART & 4.02  & 4.03  & 3.83  \\
          & mT5   & 4.18  & 4.17  & 4.05  \\
    \midrule
    \multirow{4}[2]{*}{Multi} & M-BERT & 3.89  & 3.78  & 3.70  \\
          & XLM   & \textbf{4.03 } & \textbf{3.99 } & \textbf{3.84 } \\
          & mBART & 3.96  & 3.72  & 3.58  \\
          & mT5   & 3.84  & 3.74  & 3.72  \\
    \midrule
    \multirow{4}[2]{*}{Mono-M} & M-BERT & 4.09  & 4.26  & 3.43  \\
          & XLM   & 4.12  & 4.35  & 3.38  \\
          & mBART & 4.03  & 4.19  & 3.30  \\
          & mT5   & \textbf{4.21 } & 4.35  & \textbf{3.54 } \\
    \midrule
    \multirow{4}[2]{*}{Multi-M} & M-BERT & \textbf{4.28 } & 4.33  & 3.47  \\
          & XLM   & 4.21  & 4.34  & 3.48  \\
          & mBART & 4.14  & 4.29  & 3.45  \\
          & mT5   & 4.16  & \textbf{4.43 } & \textbf{3.57 } \\
    \midrule
    \multirow{4}[2]{*}{Cross} & M-BERT & \textbf{3.82 } & \textbf{3.90 } & \textbf{3.94 } \\
          & XLM   & 3.64  & 3.64  & 3.69  \\
          & mBART & 3.68  & 3.64  & 3.70  \\
          & mT5   & 3.72  & 3.58  & 3.81  \\
    \midrule
    \multirow{4}[2]{*}{Zero} & M-BERT & 2.47  & 1.76  & 1.67  \\
          & XLM   & 3.16  & 2.69  & 2.72  \\
          & mBART & 3.31  & 3.00  & 3.18  \\
          & mT5   & \textbf{3.41 } & \textbf{3.22 } & \textbf{3.20 } \\
    \bottomrule
    \end{tabular}%
    \caption{Human evaluation on TG task under four evaluation settings. The score is 1-5 with 5 is the best. It is the average score on four languages. `Gram.', `Flu.', `Rel.' indicates \textbf{Grammar}, \textbf{Fluency} and \textbf{Relevance} respectively.}
  \label{tab:human tg}%
\end{table}%


==> tabs/mono.tex <==
% Table generated by Excel2LaTeX from sheet 'in-language'
\begin{table*}\footnotesize
\renewcommand\arraystretch{0.6}
  \centering
    \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}[0]{*}{\textbf{Task}} & \multirow{2}[0]{*}{\textbf{Model}} & \multirow{2}[0]{*}{\textbf{Language}} & \multicolumn{3}{c}{\textbf{N-gram-based}} & \multicolumn{2}{c}{\textbf{Embedding-based}} & \multicolumn{1}{c}{\textbf{Others}} \\
      &   &   & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{R-L}} & \multicolumn{1}{c}{\textbf{METEOR}} & \multicolumn{1}{c}{\textbf{BERTScore}} & \multicolumn{1}{c}{\textbf{BLEURT}} & \multicolumn{1}{c}{\textbf{D-1}} \\
    \midrule
    \multirow{8}[8]{*}{SG} & \multirow{2}[2]{*}{M-BERT} & en & 2.44 & 18.1 & 0.105 & 0.885 & -0.771 & 0.93 \\
      &   & X-Avg & 1.26 & 12.1 & 0.145 & 0.705 & - & 0.934 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{XLM} & en & 3.17 & 20.4 & 0.092 & 0.878 & -0.747 & 0.96 \\
      &   & X-Avg & 3.01 & 16.8 & 0.130 & 0.717 & - & 0.958 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mBART} & en & 4.09 & 21.4 & 0.112 & 0.894 & -0.683 & 0.98 \\
      &   & X-Avg & 3.91 & 15.9 & 0.155 & 0.742 & -  & 0.987 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mT5} & en & 1.75 & 16.6 & 0.09 & 0.886 & -0.807 & 0.98 \\
      &   & X-Avg & 1.99 & 12.2 & 0.141 & 0.728 &  - & 0.956 \\
    \midrule
    \multirow{8}[8]{*}{QG} & \multirow{2}[2]{*}{M-BERT} & en & 12.9 & 38.6 & 0.189 & 0.891 & -0.45 & 0.918 \\
      &   & X-Avg & 5.36 & 19.8 & 0.239 & 0.752 & - & 0.931 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{XLM} & en & 19.2 & 44 & 0.226 & 0.911 & -0.256 & 0.959 \\
      &   & X-Avg & 15.3 & 40.8 & 0.321 & 0.798 & - & 0.954 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mBART} & en & 19.1 & 44.7 & 0.216 & 0.912 & -0.27 & 0.971 \\
      &   & X-Avg & 14.2 & 31.6 & 0.309 & 0.802 & - & 0.98 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mT5} & en & 1.75 & 16.6 & 0.09 & 0.886 & -0.807 & 0.98 \\
      &   & X-Avg & 13.0 & 25.7 & 0.294 & 0.788 & - & 0.966 \\
    \midrule
    \multirow{8}[8]{*}{TG} & \multirow{2}[2]{*}{M-BERT} & en & 9.64 & 27.5 & 0.167 & 0.838 & -0.742 & 0.914 \\
      &   & X-Avg & 5.12 & 17.2 & 0.192 & 0.702 & - & 0.886 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{XLM} & en & 12.6 & 31.7 & 0.186 & 0.879 & \multicolumn{1}{l}{nan} & 0.96 \\
      &   & X-Avg & 8.41 & 24.3 & 0.237 & 0.732 & - & 0.915 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mBART} & en & 22.1 & 42.4 & 0.233 & 0.901 & -0.362 & 0.984 \\
      &   & X-Avg & 11.9 & 28.1 & 0.267 & 0.754 & - & 0.955 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mT5} & en & 15 & 34.7 & 0.193 & 0.888 & -0.505 & 0.975 \\
      &   & X-Avg & 8.81 & 21.1 & 0.215 & 0.727 & - & 0.946 \\
    \bottomrule
    \end{tabular}%
  \caption{Monolingual evaluation scenarios. Each model is trained and evaluated on the same language. `X-Avg' is the average score on de, fr, es. `R-L' is ROUGE-L and `D-1' is Distinct-1}
  \label{tab:mono}%
\end{table*}%






==> tabs/multi.tex <==
% Table generated by Excel2LaTeX from sheet 'in-language'
\begin{table*}\footnotesize
\renewcommand\arraystretch{0.6}
  \centering
    \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}[0]{*}{\textbf{Task}} & \multirow{2}[0]{*}{\textbf{Model}} & \multirow{2}[0]{*}{\textbf{Language}} & \multicolumn{3}{c}{\textbf{N-gram-based}} & \multicolumn{2}{c}{\textbf{Embedding-based}} & \multicolumn{1}{c}{\textbf{Others}} \\
      &   &   & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{R-L}} & \multicolumn{1}{c}{\textbf{METEOR}} & \multicolumn{1}{c}{\textbf{BERTScore}} & \multicolumn{1}{c}{\textbf{BLEURT}} & \multicolumn{1}{c}{\textbf{D-1}} \\
    \midrule
    \multirow{8}[8]{*}{SG} & \multirow{2}[2]{*}{M-BERT} & en & 2.60 & 18.1 & 0.098 & 0.888 & -0.772 & 0.971 \\
  &   & X-Avg & 1.41 & 11.9 & 0.133 & 0.714 & - & 0.974 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{XLM} & en & 2.14 & 18.3 & 0.080 & 0.874 & -0.808 & 0.964 \\
      &   & X-Avg & 2.58 & 15.9 & 0.129 & 0.714 & - & 0.964 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mBART} & en & 4.45 & 21.9 & 0.116 & 0.895 & -0.668 & 0.981 \\
      &   & X-Avg & 4.09 & 15.9 & 0.160 & 0.742 &   & 0.987 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mT5} & en & 3.77 & 20.5 & 0.108 & 0.894 & -0.700 & 0.972 \\
      &   & X-Avg & 3.43 & 15.4 & 0.152 & 0.741 &   & 0.973 \\
    \midrule
    \multirow{8}[8]{*}{QG} & \multirow{2}[2]{*}{M-BERT} & en & 14.8 & 39.2 & 0.194 & 0.891 & -0.468 & 0.918 \\
      &   & X-Avg & 6.60 & 21.5 & 0.249 & 0.754 & - & 0.937 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{XLM} & en & 19.0 & 44.4 & 0.222 & 0.910 & -0.289 & 0.955 \\
      &   & X-Avg & 15.0 & 41.1 & 0.321 & 0.799 & - & 0.953 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mBART} & en & 19.7 & 45.7 & 0.223 & 0.914 & -0.236 & 0.974 \\
      &   & X-Avg & 14.4 & 32.0 & 0.313 & 0.802 & - & 0.979 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mT5} & en & 3.77 & 20.5 & 0.108 & 0.894 & -0.700 & 0.972 \\
      &   & X-Avg & 15.9 & 33.0 & 0.330 & 0.809 & - & 0.975 \\
    \midrule
    \multirow{8}[8]{*}{TG} & \multirow{2}[2]{*}{M-BERT} & en & 9.88 & 28.1 & 0.164 & 0.848 & -0.736 & 0.931 \\
      &   & X-Avg & 5.24 & 17.4 & 0.189 & 0.703 & - & 0.906 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{XLM} & en & 12.1 & 32.2 & 0.191 & 0.880 & -0.579 & 0.956 \\
      &   & X-Avg & 8.85 & 25.5 & 0.250 & 0.730 & - & 0.907 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mBART} & en & 21.2 & 42.0 & 0.231 & 0.901 & -0.345 & 0.984 \\
      &   & X-Avg & 11.7 & 28.0 & 0.265 & 0.754 & - & 0.952 \\
    \cmidrule{2-9}  & \multirow{2}[2]{*}{mT5} & en & 17.0 & 37.1 & 0.214 & 0.893 & -0.448 & 0.976 \\
      &   & X-Avg & 10.8 & 24.6 & 0.256 & 0.743 & - & 0.936 \\
    \bottomrule
    \end{tabular}%
  \caption{Multilingual evaluation scenarios. For each task, we train the model with four languages, and directly evaluate the model on the test set of each language. `X-Avg' is the average score on de, fr, es. `R-L' is ROUGE-L and `D-1' is Distinct-1}
  \label{tab:multi}%
\end{table*}%





==> tabs/quality_check.tex <==
% Table generated by Excel2LaTeX from sheet 'quality_check'
\begin{table}[htbp]
\footnotesize
  \centering
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Tasks} & \textbf{QG} & \textbf{TG} & \textbf{SG} & \textbf{Summ} \\
    \midrule
    \textbf{German} & 0.74  & 0.7   & 0.8   & 0.68 \\
    \textbf{French} & 0.82  & 0.86  & 0.6   & 0.6 \\
    \textbf{Spanish} & 0.64  & 0.82  & 0.84  & 0.54 \\
    \textbf{Chinese} & 0.8   & 0.8   & 0.67  & 0.6 \\
    \bottomrule
    \end{tabular}%
  \caption{The quality check results of \dataset}
  \label{tab:quality check}%
\end{table}%


==> tabs/transVScross.tex <==
% Table generated by Excel2LaTeX from sheet 'transVScross'
\begin{table}[htbp]
% \footnotesize
\setlength\tabcolsep{2.5pt}
\scriptsize
  \centering
    \begin{tabular}{lccccccccccc}
    \toprule
    \textbf{Tasks} & \multicolumn{5}{c}{\textbf{SG}}       &       & \multicolumn{5}{c}{\textbf{QG}} \\
\cmidrule{1-6}\cmidrule{8-12}    \textbf{Langs} & \textbf{en} & \textbf{de} & \textbf{fr} & \textbf{es} & \textbf{zh} &       & \textbf{en} & \textbf{de} & \textbf{fr} & \textbf{es} & \textbf{zh} \\
\cmidrule{1-6}\cmidrule{8-12}    Trans & 3.26  & 3.26  & 3.26  & 3.23  & \textbf{3.71 } &       & 3.50  & 3.48  & 3.49  & 3.51  & 3.71  \\
    Cross & \textbf{3.28 } & \textbf{3.32 } & \textbf{3.34 } & \textbf{3.33 } & 3.67  &       & \textbf{3.60 } & \textbf{3.62 } & \textbf{3.63 } & \textbf{3.61 } & \textbf{3.89 } \\
    \midrule
    \textbf{Tasks} & \multicolumn{5}{c}{\textbf{TG}}       &       & \multicolumn{5}{c}{\textbf{Summ}} \\
\cmidrule{1-6}\cmidrule{8-12}    \textbf{Langs} & \textbf{en} & \textbf{de} & \textbf{fr} & \textbf{es} & \textbf{zh} &       & \textbf{en} & \textbf{de} & \textbf{fr} & \textbf{es} & \textbf{zh} \\
\cmidrule{1-6}\cmidrule{8-12}    Trans & 3.28  & 3.27  & 3.26  & 3.25  & 3.46  &       & \textbf{3.26 } & 3.25  & 3.25  & 3.26  & 2.88  \\
    Cross & \textbf{3.31 } & \textbf{3.34 } & \textbf{3.35 } & \textbf{3.34 } & \textbf{3.70 } &       & 3.22  & 3.25  & \textbf{3.29 } & \textbf{3.28 } & \textbf{3.63 } \\
    \bottomrule
    \end{tabular}%
  \caption{The ensemble metric results of trans (translate-test) and cross (crosslingual finetuned) models on the four tasks. Here every column of the subtable (lang1) represents the average score of lang1-X model results. The bold cell means the significantly better performance between trans and cross models.}
  \label{tab:transVScross}%
\end{table}%




==> tabs/transVScross_1.tex <==
% Table generated by Excel2LaTeX from sheet 'transVScross'
\begin{table}[htbp]
% \footnotesize
\setlength\tabcolsep{2.5pt}
\scriptsize
  \centering
    \begin{tabular}{lccccccccccc}
    \toprule
    \textbf{Tasks} & \multicolumn{5}{c}{\textbf{SG}}       &       & \multicolumn{5}{c}{\textbf{QG}} \\
\cmidrule{1-6}\cmidrule{8-12}    \textbf{Langs} & \textbf{en} & \textbf{de} & \textbf{fr} & \textbf{es} & \textbf{zh} &       & \textbf{en} & \textbf{de} & \textbf{fr} & \textbf{es} & \textbf{zh} \\
\cmidrule{1-6}\cmidrule{8-12}    zero  & 3.26  & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} &       & 3.50  & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} \\
    Trans & 3.26  & 3.26  & 3.26  & 3.23  & \textbf{3.71 } &       & 3.50  & 3.48  & 3.49  & 3.51  & 3.71  \\
    Cross & \textbf{3.28 } & \textbf{3.32 } & \textbf{3.34 } & \textbf{3.33 } & 3.67  &       & \textbf{3.60 } & \textbf{3.62 } & \textbf{3.63 } & \textbf{3.61 } & \textbf{3.89 } \\
    \midrule
    \textbf{Tasks} & \multicolumn{5}{c}{\textbf{TG}}       &       & \multicolumn{5}{c}{\textbf{Summ}} \\
\cmidrule{1-6}\cmidrule{8-12}    \textbf{Langs} & \textbf{en} & \textbf{de} & \textbf{fr} & \textbf{es} & \textbf{zh} &       & \textbf{en} & \textbf{de} & \textbf{fr} & \textbf{es} & \textbf{zh} \\
\cmidrule{1-6}\cmidrule{8-12}    zero  & 3.28  & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} &       & 3.26  & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} \\
    Trans & 3.28  & 3.27  & 3.26  & 3.25  & 3.46  &       & 3.26  & 3.25  & 3.25  & 3.26  & 2.88  \\
    Cross & \textbf{3.31 } & \textbf{3.34 } & \textbf{3.35 } & \textbf{3.34 } & \textbf{3.70 } &       & 3.22  & 3.25  & \textbf{3.29 } & \textbf{3.28 } & \textbf{3.63 } \\
    \bottomrule
    \end{tabular}%
  \caption{The ensemble metric results of zero (zero-shot), trans (translation-test) and cross (crosslingual finetuned) models on the four tasks. Here every column of the subtable (lang1) represents the average score of lang1-X model results. The bold cell means the better performance between trans and cross models.}
  \label{tab:transVScross}%
\end{table}%




==> tabs/zero.tex <==
% Table generated by Excel2LaTeX from sheet 'Cross-lingual'
\begin{table}\footnotesize
\renewcommand\arraystretch{0.9}
  \centering
    \begin{tabular}{clccc}
    \toprule
    \textbf{Task} & \multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{R-L}} & \multicolumn{1}{c}{\textbf{BERTScore}} & \multicolumn{1}{c}{\textbf{D-1}} \\
    \midrule
    \multirow{4}[2]{*}{SG} & M-BERT & 3.20 & 0.703 & 0.941 \\
      & XLM & 9.07 & 0.687 & 0.892 \\
      & mBART & 3.96 & 0.687 & 0.904 \\
      & mT5 & 3.27 & 0.706 & 0.980 \\
    \midrule
    \multirow{4}[2]{*}{QG} & M-BERT & 3.10 & 0.748 & 0.924 \\
      & XLM & 19.6 & 0.739 & 0.936 \\
      & mBART & 5.35 & 0.745 & 0.976 \\
      & mT5 & 4.85 & 0.748 & 0.971 \\
    \midrule
    \multirow{4}[2]{*}{TG} & M-BERT & 7.17 & 0.658 & 0.907 \\
      & XLM & 13.7 & 0.688 & 0.883 \\
      & mBART & 13.3 & 0.711 & 0.973 \\
      & mT5 & 11.2 & 0.701 & 0.969 \\
    \bottomrule
    \end{tabular}%
    \caption{Zero-shot tranfer scenarios. The notations are the same with Table \ref{tab:cross}.}
  \label{tab:zero}%
\end{table}%



==> tabs/zeroVScross.tex <==
% Table generated by Excel2LaTeX from sheet 'transVScross'
\begin{table}[htbp]
  \centering
  \footnotesize
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Tasks} & \textbf{SG} & \textbf{QG} & \textbf{TG} & \textbf{Summ} \\
    \midrule
    Zero  & 3.26  & 3.50  & 3.28  & \textbf{3.26 } \\
    Cross & \textbf{3.28 } & \textbf{3.60 } & \textbf{3.31 } & 3.22  \\
    \bottomrule
    \end{tabular}%
    \caption{The average model performance in zero-shot and cross-lingual setting.}
  \label{tab:zero vs cross}%
\end{table}%


==> tabs/zero_TG.tex <==
% Table generated by Excel2LaTeX from sheet 'zeroshot_en'
\begin{table*}[htbp]
  \centering
  \footnotesize
  \renewcommand\arraystretch{0.87}
  \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{clccccccccc}
    \toprule
    \textbf{Model} & \multicolumn{1}{c}{\textbf{Language}} & \textbf{BLEU} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{D-1} & \textbf{D-2} & \textbf{Ensemble} \\
    \midrule
    \multirow{4}[2]{*}{mbert} & en->de & 5.14  & 12.4  & 4.1   & 11.8  & 0.136 & 0.697 & 0.928 & 0.988 & 31.8 \\
          & en->fr & 3.6   & 11.4  & 3.3   & 10.8  & 0.117 & 0.702 & 0.936 & 0.989 & 28.9 \\
          & en->es & 3.76  & 10.9  & 3.3   & 10.4  & 0.142 & 0.711 & 0.928 & 0.988 & 28.5 \\
          & en->zh & 0.56  & 2.1   & 0.5   & 2.1   & -     & 0.557 & 0.928 & 0.988 & 21.7 \\
    \midrule
    \multirow{4}[2]{*}{xlm} & en->de & 2.58  & 13.4  & 4.4   & 12.5  & 0.12  & 0.665 & 0.83  & 0.877 & 26.3 \\
          & en->fr & 3.26  & 13.9  & 4.5   & 12.7  & 0.12  & 0.685 & 0.887 & 0.933 & 25.2 \\
          & en->es & 4.9   & 21.2  & 7.4   & 18.5  & 0.169 & 0.705 & 0.875 & 0.936 & 24.5 \\
          & en->zh & 0.01  & 0     & 0     & 0     & -     & 0.446 & 0.372 & 0.224 & 16.7 \\
    \midrule
    \multirow{4}[2]{*}{mbart} & en->de & 5.49  & 14.9  & 5.7   & 14.4  & 0.142 & 0.706 & 0.983 & 0.999 & 32.2 \\
          & en->fr & 3.79  & 13.2  & 4.4   & 12.6  & 0.118 & 0.713 & 0.988 & 1     & 28.9 \\
          & en->es & 3.89  & 12.9  & 4.4   & 12.3  & 0.149 & 0.721 & 0.983 & 0.999 & 29.7 \\
          & en->zh & 0.71  & 2.9   & 0.7   & 2.9   & -     & 0.56  & 0.983 & 0.999 & 22.6 \\
    \midrule
    \multirow{4}[2]{*}{mt5} & en->de & 5.41  & 13.5  & 5.2   & 12.9  & 0.133 & 0.696 & 0.974 & 0.996 & 31.9 \\
          & en->fr & 4.04  & 12.2  & 4.1   & 11.5  & 0.112 & 0.703 & 0.979 & 0.997 & 29.1 \\
          & en->es & 4.09  & 11.9  & 4.1   & 11.3  & 0.138 & 0.712 & 0.975 & 0.996 & 29.7 \\
          & en->zh & 0.79  & 2.5   & 0.6   & 2.4   & -     & 0.553 & 0.973 & 0.995 & 21.9 \\
    \bottomrule
    \end{tabular}%
    }
   \caption{Zero shot results for four models on title generation. Here R-* and D-* represent ROUGE-* and Distant-* respectively.}
  \label{tab:zeroshot TG}%
\end{table*}%




==> tabs/zero_all.tex <==
% % Table generated by Excel2LaTeX from sheet 'zero_shot'
% \begin{table*}[htbp]
%   \centering
%   \footnotesize
%   \renewcommand\arraystretch{0.9}
%     \begin{tabular}{clccccccccc}
%     \toprule
%     \textbf{Setting} & \multicolumn{1}{c}{\textbf{Model}} & \textbf{BLEU} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{D-1} & \textbf{D-2} & \textbf{Ensemble} \\
%     \midrule
%     \multirow{4}[2]{*}{SG} & M-BERT & 0.0   & 3.2   & 0.0   & 3.2   & 0.048  & 0.703  & 0.94  & 0.98  & 2.746  \\
%           & XLM   & 0.5   & 9.6   & 1.1   & 9.1   & 0.068  & 0.694  & 0.89  & 0.92  & 3.074  \\
%           & mBART & 0.1   & 4.0   & 0.0   & 4.0   & 0.038  & 0.687  & 0.90  & 0.98  & 2.458  \\
%           & mT5   & 0.1   & 3.3   & 0.0   & 3.3   & 0.044  & 0.705  & 0.98  & 1.00  & 2.768  \\
%     \midrule
%     \multirow{4}[2]{*}{QG} & M-BERT & 0.6   & 3.2   & 0.4   & 3.1   & 0.059  & 0.731  & 0.92  & 0.99  & 2.636  \\
%           & XLM   & 2.9   & 20.7  & 4.1   & 19.6  & 0.126  & 0.738  & 0.94  & 0.98  & 3.297  \\
%           & mBART & 1.0   & 5.5   & 1.0   & 5.3   & 0.071  & 0.745  & 0.98  & 1.00  & 2.820  \\
%           & mT5   & 1.3   & 5.0   & 1.0   & 4.9   & 0.075  & 0.748  & 0.97  & 1.00  & 2.838  \\
%     \midrule
%     \multirow{4}[2]{*}{TG} & M-BERT & 2.0   & 7.5   & 2.0   & 7.2   & 0.106  & 0.658  & 0.91  & 0.95  & 3.007  \\
%           & XLM   & 3.4   & 14.9  & 5.2   & 13.7  & 0.133  & 0.688  & 0.88  & 0.93  & 3.150  \\
%           & mBART & 4.5   & 13.9  & 5.1   & 13.3  & 0.145  & 0.711  & 0.97  & 1.00  & 3.222  \\
%           & mT5   & 4.4   & 11.8  & 4.3   & 11.2  & 0.128  & 0.686  & 0.97  & 0.99  & 3.135  \\
%     \bottomrule
%     \end{tabular}%
%     \caption{Zero shot results for four models on three tasks. The results are the average scores on the en->de, en->fr, en->es test set. Here R-* and D-* represent ROUGE-* and Distant-* respectively.}
%   \label{tab:zero_all}%
% \end{table*}%

% Table generated by Excel2LaTeX from sheet 'zeroshot_en'
\begin{table*}[htbp]
  \centering
  \footnotesize
  \renewcommand\arraystretch{0.87}
  \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{clccccccccc}
    \toprule
    \textbf{Setting} & \textbf{Model} & \textbf{BLEU} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{D-1} & \textbf{D-2} & \textbf{Ensemble} \\
    \midrule
    \multirow{4}[2]{*}{SG} & M-BERT & 0.04  & 2.73  & 0.00  & 2.70  & 0.04  & 0.66  & 0.92  & 0.99  & 3.63  \\
          & XLM   & 0.03  & 5.45  & 0.20  & 5.40  & 0.04  & 0.59  & 0.49  & 0.51  & 3.10  \\
          & mBART & 0.06  & 3.18  & 0.00  & 3.18  & 0.05  & 0.67  & 0.98  & 1.00  & 3.76  \\
          & mT5   & 0.04  & 2.08  & 0.00  & 2.05  & 0.04  & 0.67  & 0.98  & 1.00  & 3.77  \\
    \midrule
    \multirow{4}[2]{*}{QG} & M-BERT & 0.43  & 2.68  & 0.38  & 2.63  & 0.06  & 0.69  & 0.91  & 0.99  & 3.50  \\
          & XLM   & 2.90  & 15.10  & 3.50  & 14.43  & 0.12  & 0.67  & 0.73  & 0.76  & 2.99  \\
          & mBART & 0.91  & 6.35  & 0.78  & 6.20  & 0.07  & 0.70  & 0.98  & 1.00  & 3.59  \\
          & mT5   & 0.97  & 3.83  & 0.73  & 3.73  & 0.07  & 0.70  & 0.97  & 1.00  & 3.57  \\
    \midrule
    \multirow{4}[2]{*}{TG} & M-BERT & 3.27  & 9.20  & 2.80  & 8.78  & 0.13  & 0.67  & 0.93  & 0.99  & 3.52  \\
          & XLM   & 2.69  & 12.13  & 4.08  & 10.93  & 0.14  & 0.63  & 0.74  & 0.74  & 2.90  \\
          & mBART & 3.47  & 10.98  & 3.80  & 10.55  & 0.14  & 0.68  & 0.98  & 1.00  & 3.64  \\
          & mT5   & 3.58  & 10.03  & 3.50  & 9.53  & 0.13  & 0.67  & 0.98  & 1.00  & 3.61  \\
    \midrule
    \multirow{4}[2]{*}{Summ} & M-BERT & 1.29  & 7.40  & 1.38  & 7.15  & 0.08  & 0.65  & 0.82  & 0.98  & 3.53  \\
          & XLM   & 1.83  & 12.90  & 2.83  & 11.95  & 0.10  & 0.61  & 0.64  & 0.67  & 2.82  \\
          & mBART & 0.05  & 5.50  & 1.48  & 5.38  & 0.04  & 0.62  & 0.96  & 1.00  & 3.19  \\
          & mT5   & 0.59  & 5.93  & 1.20  & 5.70  & 0.05  & 0.63  & 0.84  & 0.94  & 3.20  \\
    \bottomrule
    \end{tabular}%
    }
  \caption{Zero shot results for four models on four tasks. The results are the average scores on the en->de, en->fr, en->es test set. Here R-* and D-* represent ROUGE-* and Distant-* respectively.}
  \label{tab:zero_all}%
\end{table*}%



==> tabs/zero_v2.tex <==
% Table generated by Excel2LaTeX from sheet 'zeroshot_en'
\begin{table*}[htbp]
  \centering
  \footnotesize
  \renewcommand\arraystretch{0.87}
  \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{clccccccccc}
    \toprule
    \textbf{Task} & \multicolumn{1}{c}{\textbf{Model}} & \textbf{BLEU} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{METEOR} & \textbf{BERTScore} & \textbf{D-1} & \textbf{D-2} & \textbf{Ensemble} \\
    \midrule
    \multirow{4}[2]{*}{SG} & mbert & 0.04  & 2.73  & 0.00  & 2.70  & 0.04  & 0.66  & 0.92  & 0.99  & 29.65  \\
          & xlm   & 0.03  & 5.45  & 0.20  & 5.40  & 0.04  & 0.59  & 0.49  & 0.51  & 16.67  \\
          & mbart & 0.06  & 3.18  & 0.00  & 3.18  & 0.05  & 0.67  & 0.98  & 1.00  & 29.62  \\
          & mt5   & 0.04  & 2.08  & 0.00  & 2.05  & 0.04  & 0.67  & 0.98  & 1.00  & 29.81  \\
    \midrule
    \multirow{4}[2]{*}{QG} & mbert & 0.43  & 2.68  & 0.38  & 2.63  & 0.06  & 0.69  & 0.91  & 0.99  & 28.45  \\
          & xlm   & 2.90  & 15.10  & 3.50  & 14.43  & 0.12  & 0.67  & 0.73  & 0.76  & 25.82  \\
          & mbart & 0.91  & 6.35  & 0.78  & 6.20  & 0.07  & 0.70  & 0.98  & 1.00  & 26.97  \\
          & mt5   & 0.97  & 3.83  & 0.73  & 3.73  & 0.07  & 0.70  & 0.97  & 1.00  & 28.42  \\
    \midrule
    \multirow{4}[2]{*}{TG} & mbert & 3.27  & 9.20  & 2.80  & 8.78  & 0.13  & 0.67  & 0.93  & 0.99  & 27.75  \\
          & xlm   & 2.69  & 12.13  & 4.08  & 10.93  & 0.14  & 0.63  & 0.74  & 0.74  & 23.18  \\
          & mbart & 3.47  & 10.98  & 3.80  & 10.55  & 0.14  & 0.68  & 0.98  & 1.00  & 28.36  \\
          & mt5   & 3.58  & 10.03  & 3.50  & 9.53  & 0.13  & 0.67  & 0.98  & 1.00  & 28.15  \\
    \midrule
    \multirow{4}[2]{*}{Summ} & mbert & 1.29  & 7.40  & 1.38  & 7.15  & 0.08  & 0.65  & 0.82  & 0.98  & 20.78  \\
          & xlm   & 1.83  & 12.90  & 2.83  & 11.95  & 0.10  & 0.61  & 0.64  & 0.67  & 16.82  \\
          & mbart & 1.27  & 7.73  & 1.55  & 7.48  & 0.07  & 0.65  & 0.85  & 0.99  & 20.17  \\
          & mt5   & 0.59  & 5.93  & 1.20  & 5.70  & 0.05  & 0.63  & 0.84  & 0.94  & 16.80  \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Zero shot results for four models on three tasks. The results are the average scores on the en->de, en->fr, en->es test set. Here R-* and D-* represent ROUGE-* and Distant-* respectively.}
  \label{tab:zeroshot}%
\end{table*}%



